The Satisfiability and Validity Problems for Probabilistic Computational Tree Logic are Highly Undecidable

The Probabilistic Computational Tree Logic (PCTL) is the main specification formalism for discrete probabilistic systems modeled by Markov chains. Despite serious research attempts, the decidability of PCTL satisfiability and validity problems remained unresolved for 30 years. We show that both problems are highly undecidable, i.e., beyond the arithmetical hierarchy. Consequently, there is no sound and complete deductive system for PCTL.

==> conclusions.tex <==
\section{Conclusions}
\label{sec-concl}

We have shown that the general/finite PCTL satisfiability problems are undecidable. 
Note that the formula $\Psi$ constructed in the proof of Theorem~\ref{thm-two-counter} is \emph{always} generally satisfiable, which implies that the finite satisfiability problem for PCTL is undecidable even for the subset of generally satisfiable PCTL formulae. Furthermore, the undecidability result remains valid even if the set of eligible finite models is restricted to \emph{tree-like} models, where the underlying graph of a Markov chain is a tree with self-loops on all leaves (this requires a slight modification of our construction).
Finally, let us note that the construction of Theorem~\ref{thm-two-counter} applies also to a universal Minsky machine. Hence, fixed parameterized PCTL formulae exist such that the general/finite satisfiability of their instances is undecidable. 

==> counter.tex <==
\section{Simulating Minsky machines with one counter}
\label{sec-counter}

For the rest of this section, we fix $q$, $I_q$, and $\vec{\kappa}$ in the same way as in Section~\ref{sec-geom}, but we additionally require that $\vec{\kappa}_1 + \vec{\kappa}_2 < q - \frac{1}{2}$. Furthermore, we fix a rational constant  $\gamma$ such that $(1{-}q) \vec{\kappa}_2 < \gamma < \frac{3}{4}q - \frac{5}{4}q + \frac{1}{2}q^2$. For example, we can put $q = \frac{13}{16}$, $\vec{\kappa}= (\frac{17}{64},\frac{1}{32})$, and $\gamma = 0.06$.
These additional assumptions are used in the proof of Theorem~\ref{thm-one-counter}.


Let $\M$ be a non-deterministic one-counter Minsky machine with $m$ instructions, and let $\Labels = \{\ell_i \mid 1\leq i \leq m\}$ be a set of fresh atomic propositions. Let $M = (S,P,v)$ be a Markov chain. We say that a state $t \in S$ \emph{represents a configuration $(i,n)$} of $\M$ iff $t \models \ell_i$, $t \not\models \ell_j$ for all $j \neq i$, and $\vec{v}[t] = \sigma^n(\vec{\kappa})$. Furthermore, we say that a state $s \in S$ \emph{simulates $\M$} if $s$ represents $(1,0)$ and every state $t$ reachable from $s$ satisfies the following condition: If $t$ represents a configuration $C$ of $\M$, then at least one immediate successor of $t$ represents a successor configuration of~$C$. Furthermore, for every immediate successor $t'$ of $t$ that does \emph{not} represent a successor of $C$ we have that $t' \models \opg_{=1} \bigwedge_{i=1}^m \neg\ell_i$.

% one of the following conditions:
% \begin{itemize}
%     \item $t$ and all immediate successors of $t$ satisfy $\bigwedge_{i=1}^m \neg\ell_i$.
%     \item $t$ represents a configuration $C$ of $\M$, and at least one immediate successor of $t$ represents a successor configuration of~$C$. Furthermore, for every immediate successor $t'$ of $t$ that does \emph{not} represent a successor of $C$ we have that $t'$ satisfies $\bigwedge_{i=1}^m \neg\ell_i$.
% \end{itemize}
Let $s \in S$ be a state simulating $\M$, and let $s_0,s_1,\ldots$ be a run such that $s_0 = s$ and every $s_i$ represents a configuration $C_i$ of $\M$. Then $C_0,C_1,\ldots$ is a computation of $\M$ \emph{covered by $s$}. Note that $s$ covers at least one but not necessarily all computations of~$\M$.
%
In this section, we prove the following theorem:

\begin{theorem}
\label{thm-one-counter}
Let $\M$ be a non-deterministic one-counter Minsky machine. Then there is an effectively constructible PCTL formula $\psi$ satisfying the following conditions:
\begin{itemize}
    \item[(A)] For every Markov chain $M$ and every state $s$ of $M$, we have that if $s \models \psi$, then $s$ simulates $\M$.
    \item[(B)] For every computation $\omega$ of $\M$, there exists a Markov chain $M$ and a state $s$ of $M$ such that $s \models \psi$ and $s$ covers $\omega$. 
    Furthermore, if $\omega$ is periodic, then $M$ has finitely many states.
\end{itemize}
\end{theorem}

% For the rest of this section, we fix a non-deterministic one-counter Minsky machine 
% $\M \ \equiv\ 1: \Ins_1; \ \cdots  \ m: \Ins_m;$ 

% In Section~\ref{sec-one-counter-psi}, we show how to construct the formula $\psi$ for $\M$. Recall that the counter values $0,1,2,\ldots$ are represented by characteristic vectors $\vec{\kappa}$, $\sigma(\vec{\kappa})$, $\sigma^2(\vec{\kappa}),\ldots$. Hence, decrementing and incrementing the counter corresponds to performing the functions $\tau$ and $\sigma$, respectively. Testing the counter for zero is no issue because both components of $\vec{\kappa}$ are rational and can be directly used as probability constraints. The function $\tau$ is implemented in the same way as in the parameterized formula $\psi(x,y)$ constructed in Section~\ref{sec-large}. Consequently, some subformulae of $\psi(x,y)$ are re-used in~$\psi$, possibly after small adjustments. The main challenge is to implement the function~$\sigma$ and orchestrate everything so that Theorem~\ref{thm-area} is still applicable.

% %To simplify the construction of $\psi$, we adopt the technical assumptions about $\M$ formulated in Section~\ref{sec-Minsky}.

% % Furthermore, we fix $q$, $I_q$, and $\vec{\kappa}$ in the same way as in Section~\ref{sec-large}, but we additionally require that $\vec{\kappa}_1 + \vec{\kappa}_2 < q - \frac{1}{2}$. Finally, we fix a rational constant $\gamma$ such that $(1{-}q) \vec{\kappa}_2 < \gamma < \frac{3}{4}q - \frac{5}{4}q + \frac{1}{2}q^2$. For example, we can put $q = \frac{13}{16}$, $\vec{\kappa}= (\frac{17}{64},\frac{1}{32})$, and $\gamma = 0.06$.
% % These additional assumptions are used in the proofs of Proposition~\ref{prop-one-counter-bounded} and Proposition~\ref{prop-Minsky-bounded}.


% Intuitively, the counter values $0,1,2,\ldots$ are represented by characteristic vectors $\vec{\kappa}$, $\sigma(\vec{\kappa})$, $\sigma^2(\vec{\kappa}),\ldots$. Hence, decrementing and incrementing the counter corresponds to performing the functions $\tau$ and $\sigma$, respectively. Testing the counter for zero is no issue because both components of $\vec{\kappa}$ are rational and can be directly used as probability constraints. The function $\tau$ is implemented in the same way as in the parameterized formula $\psi(x,y)$ constructed in Section~\ref{sec-large}. Consequently, some subformulae of $\psi(x,y)$ are re-used in~$\psi$, possibly after small adjustments. The main challenge is to implement the function~$\sigma$ and orchestrate everything so that Theorem~\ref{thm-area} is still applicable.

\subsection{Constructing $\psi$}
\label{sec-one-counter-psi}

For the rest of this section, we fix a non-deterministic one-counter Minsky machine 
$\M \ \equiv\ 1: \Ins_1; \ \cdots  \ m: \Ins_m$. We show how to construct the formula $\psi$ of Theorem~\ref{thm-one-counter}.

Recall that the counter values $0,1,2,\ldots$ are represented by characteristic vectors $\vec{\kappa}$, $\sigma(\vec{\kappa})$, $\sigma^2(\vec{\kappa}),\ldots$. Hence, decrementing and incrementing the counter corresponds to performing the functions $\tau$ and $\sigma$, respectively. Testing the counter for zero is no issue because both components of $\vec{\kappa}$ are rational and can be directly used as probability constraints. The function $\tau$ is implemented in the same way as in the parameterized formula $\psi(x,y)$ constructed in Section~\ref{sec-large}. Consequently, some subformulae of $\psi(x,y)$ are re-used in~$\psi$, possibly after small adjustments. The main challenge is to implement the function~$\sigma$ and orchestrate everything so that Theorem~\ref{thm-area} is still applicable.

The set of propositions used in $\psi$ is $\A = A \cup \Labels \cup \{d,e\}$ where $A$ is the set of propositions occurring in $\psi(x,y)$ (see Section~\ref{sec-large}), and $d,e$ are fresh propositions used for implementing the function $\sigma$. For every $B \subseteq \A$, we use $\Ex{B}$ to denote the formula  $\bigwedge_{p \in B} p \wedge \bigwedge_{p \in \A \smallsetminus B} \neg p$. The intuitive meaning of $\Ex{B}$ is the same as of $\ex{B}$ defined in Section~\ref{sec-large-formula}. The only difference is that the set $A$ is replaced with the richer set~$\A$. 

The structure of $\psi$ closely resembles the structure of $\psi(x,y)$, and the overall intuition behind the subformulae stays essentially the same. We use the same identifiers for denoting adjusted versions of subformulae defined in Section~\ref{sec-large-formula}. If a subformula does not require any adjustment \emph{except for replacing every occurrence of $\ex{\cdot}$ with $\Ex{\cdot}$}, then we re-use this formula and write its identifier in \textit{\textbf{boldface}}. For example, $\bFsuc_i$ denotes the formula
\[
  \opx_{=1} (\Ex{h,a,S(r_i)} \vee \Ex{h,b,S^2(r_i)} \vee \Ex{h,c,S^2(r_i)})\,.   
\]

We put 
\begin{eqnarray*}
     \psi & \equiv &  \Init \ \wedge \ \opg_{=1} \Invariant   
\end{eqnarray*}
where
\begin{eqnarray*}
    \Init & \equiv & \Ex{a,r_0,\ell_1} \ \wedge \ \bZero\\
    \Invariant & \equiv & \bFin \vee \Transient \vee \bFree
\end{eqnarray*}
Note that if $s \models \psi$, then every state $t$ reachable form $s$ can again be classified as either \emph{final}, \emph{transient}, or \emph{free}, depending on whether $t$~satisfies $\bFin$, $\Transient$, or $\bFree$, respectively.  

%
% The formula $\Init$ says that the counter is initially zero and $\Ins_1$ will be simulated next. The formulae $\Free$ and $\Final$ are defined in the same way as $\bFree$ and $\bFinal$, except for using $\Ex{\cdot}$ instead of $\ex{\cdot}$.
% \begin{eqnarray*}
%     \Free & \equiv & h \wedge \bigvee_{B \subseteq \A} (\Ex{B} \wedge \opx_{=0} \neg \Ex{B})\\
%     \Final & \equiv & \bigvee_{i \in \{0,\ldots,4\}} \Ex{a,r_i} \wedge \bFsuc_i \wedge \bZero 
% \end{eqnarray*}
% The formula $\Final$ is defined as follows:
% % \[
% %     \Final \ \equiv \ \bFin \ \vee \ \bigvee_{i \in \{0,\ldots,4\}} (r_i \wedge \ell_{m{+}1} \wedge \bFsuc_i) 
% % \]
% \[
%     \Final \ \equiv \ \bigvee_{i \in \{0,\ldots,4\}} \Ex{a,r_i} \wedge \bFsuc_i \wedge \bZero 
% \]
% Thus, the set of final states is extended with the set of states simulating the $\Halt$ instruction of $\M$. Recall that the counter is zero when $\M$ reaches $\Halt$ (see Section~\ref{sec-Minsky}). 
%
Furthermore, we put
\[
    \Transient \ \equiv \ \bTrans \vee \CTrans \vee \LTrans \,.
\]   
As we shall see, every transient state $t$ satisfies precisely one of the formulae $\Ex{a,r_i}$, $c {\wedge} r_i {\wedge} \neg h$, or $\Ex{x,r_i,\ell}$, where $i \in \{0,\ldots,4\}$, \mbox{$\ell \in \Labels$}, and $x \in \{a,b\}$. The formulae $\bTrans$, $\CTrans$, and $\LTrans$ define the properties of~$t$ in the three respective cases. We define
\begin{eqnarray*}
    % \ATrans & \equiv & \bigvee_{i \in \{0,\ldots,4\}} \Ex{a,r_i} \wedge \bSuc_i \wedge \bInterval \wedge \bEq_i\\
    \CTrans &\equiv & \bigvee_{i \in \{0,\ldots,4\}} c \wedge r_i \wedge \neg h \wedge \Csuc_i \wedge \bInterval \wedge \bEq_i   
\end{eqnarray*}
where
\[
    \Csuc_i \equiv  \opx_{=1} \big( \Ex{a,S(r_i)} \vee \Ex{h,b,S^2(r_i)}
     \vee \ \Ex{h,c,S^2(r_i)}  \vee  \Ex{h,c,S^2(r_i),d} \big)  
\]
% \begin{eqnarray*}
%    \Csuc_i & \equiv & \opx_{=1} \big( \Ex{a,S(r_i)} \vee \Ex{h,b,S^2(r_i)}\\
%    && \hspace*{5ex} \vee \ \Ex{h,c,S^2(r_i)}  \vee  \Ex{h,c,S^2(r_i),d} \big)  
% \end{eqnarray*}
Furthermore, we define 
\begin{eqnarray*}   
    \LTrans & \equiv &\bigvee_{i \in \{0,\ldots,4\}} \bigvee_{\ell \in \Labels} \bigvee_{x \in \{a,b\}} 
    \  (\Ex{x,r_i,\ell} \wedge \Step_{i,\ell})
\end{eqnarray*}
where the formula $\Step_{i,\ell}$ is constructed as follows. Let $\Ins_j$ be the instruction associated with $\ell$, i.e., $\ell = \ell_j$. We distinguish two cases.
\bigskip

\noindent 
(A)  If $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } L \textit{ else dec } c; \textit{ goto } L'$, then
    \begin{eqnarray*}
        \Step_{i,\ell} & \equiv & \hspace*{2ex} \left(\bZero \Rightarrow (\Zsuc_{i,\ell} \wedge \opx_{=1} (b \Rightarrow \bZero))\right)\\
        && \wedge \left( \neg\bZero \Rightarrow (\Psuc_{i,\ell} \wedge \bInterval \wedge \bEq_i ) \right)
    \end{eqnarray*}
    where 
    \begin{eqnarray*}
        \Zsuc_{i,\ell} & \equiv & \bigvee_{\ell' \in L} \opx_{=1} \big(\Ex{h,a,S(r_i)} \vee \Ex{h,c,S^2(r_i)} \vee \Ex{h,c,S^2(r_i),e}\\[-3ex]       
        && \hspace*{9ex} \vee~  \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ 
            \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e}\\
%
    %    \Zsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)} \vee \Ex{h,c,S^2(r_i)} \vee \Ex{h,c,S^2(r_i),e}\\       
    %     && \hspace*{5ex} \vee \bigvee_{\ell' \in L} \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e}\\
        \Psuc_{i,\ell} & \equiv & \bigvee_{\ell' \in L'} \opx_{=1} \big(\Ex{h,b,S^2(r_i)} \vee \Ex{h,c,S^2(r_i)} \vee \Ex{h,c,S^2(r_i),e}\\[-3ex]
        &&  \hspace*{9ex} \vee~  \Ex{a,S(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e}  
        % \Psuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{h,b,S^2(r_i)} \vee \Ex{h,c,S^2(r_i)} \vee \Ex{h,c,S^2(r_i),e}\\
        % &&  \hspace*{5ex} \vee \bigvee_{\ell' \in L'} \Ex{a,S(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e}  
    \end{eqnarray*}
    % and 
    % \begin{eqnarray*}
    %     \Psuc_{i,\ell,a} & \equiv & \opx_{=1} \big(\Ex{a,S(r_i),\ell_{u'}} \vee \Ex{h,b,S^2(r_i)} \vee \Ex{h,c,S^2(r_i)} \big)\\
    %     \Psuc_{i,\ell,b} & \equiv & \opx_{=1} \big(\Ex{a,S(r_i),\ell_{u'}} \vee \Ex{h,b,S^2(r_i)} \vee \Ex{h,c,S^2(r_i)}\\
    %     &&  \hspace*{5ex} \vee \Ex{h,c,S^2(r_i),e} \big) \ \wedge \ \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e} 
    % \end{eqnarray*} 
\noindent
(B) If $\Ins_j \equiv \textit{inc } c; \textit{ goto } L$, then
\begin{eqnarray*}
    \Step_{i,\ell} & \equiv & 
    \hspace*{2ex} (\bZero \Rightarrow \IZsuc_{i,\ell})\\
    && \wedge \ (\neg\bZero \Rightarrow (\IPsuc_{i,\ell} \wedge \bInterval \wedge \bEq_i)\\
    && \wedge \ \opf^2_{=1{-}q} (a\wedge S^3(r_i))\\
    && \wedge \ \opf^2_{=\gamma} \big((b \wedge S^4(r_i) ) \vee d\big)\\
    && \wedge \ \opf^2_{=\gamma} \big((c\wedge S^4(r_i) \wedge e) \vee d \big)
\end{eqnarray*}
where $\gamma$ is the constant fixed at the beginning of Section~\ref{sec-counter} and
\begin{eqnarray*}
    % \IZsuc_{i,\ell,a} & \equiv & \opx_{=1} \big( \Ex{h,a,S(r_i)} \vee \Ex{b,S^2(r_i),\ell_u} \vee
    % \Ex{c,S^2(r_i)} \big)\\
    % \IPsuc_{i,\ell,a} & \equiv & \opx_{=1} \big( \Ex{a,S(r_i)} \vee \Ex{b,S^2(r_i),\ell_u} \vee
    % \Ex{c,S^2(r_i)} \big)\\
    \IZsuc_{i,\ell} & \equiv & \bigvee_{\ell' \in L} \opx_{=1} \big(\Ex{h,a,S(r_i)}  \vee
    \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\[-3ex]
    && \hspace*{9ex}  \vee~  \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}\\
%
    % \IZsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)}  \vee
    % \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\
    % && \hspace*{5ex}  \vee \bigvee_{\ell' \in L} \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}\\
    \IPsuc_{i,\ell} & \equiv & \bigvee_{\ell' \in L} \opx_{=1} \big(\Ex{a,S(r_i)}  \vee
    \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\[-3ex]
    && \hspace*{9ex}  \vee~  \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}
    % \IPsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{a,S(r_i)}  \vee
    % \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\
    % && \hspace*{5ex}  \vee \bigvee_{\ell' \in L} \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}
\end{eqnarray*}
%
This completes the construction of $\psi$.

Intuitively, if $t \models \Ex{x,r_i,\ell_j}$ and $\vec{v}[t]$ encodes the current counter value, then $\Step_{i,\ell_j}$ enforces the simulation of $\Ins_j$. More concretely,  
\begin{itemize}
    \item if $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } L \textit{ else dec } c; \textit{ goto } L'$, then 
    \begin{itemize}
        \item if $\vec{v}[t] = \vec{\kappa}$ encodes zero, then each $t' \in \Bs{t}$ satisfies some $\ell' \in L$ and $\vec{v}[t']= \vec{\kappa}$. The simulation continues in the states of~$\Bs{t}$.
        \item if $\vec{v}[t]$ encodes a positive value, then each $t' \in \As{t}$ satisfies some $\ell' \in L'$ and $\vec{v}[t'] = \tau(\vec{v}[t])$. The counter is decremented, and the simulation continues in the states of~$\As{t}$.
    \end{itemize}
    \item If $\Ins_j \equiv \textit{inc } c; \textit{ goto } L$, then each $t' \in \Bs{t}$ satisfies some $\ell' \in L$. Furthermore, $\vec{v}[t'] = \sigma(\vec{v}[t])$ for all $t' \in \Bs{t} \cup \Cs{t}$ (this part is tricky). The counter is incremented and the simulation continues in the states of $\Bs{t}$. %The reason why $\vec{v}[t'] = \sigma(\vec{v}[t])$ also for $t' \in \Cs{t}$ is clarified in Section~\ref{sec-prop-one-counter-unbounded}.
\end{itemize}
Furthermore, all transient states~$t$ where $\vec{v}[t] \neq \vec{\kappa}$ satisfy the formula $\bInterval \wedge \bEq_i$ (for an appropriate $i$) so that the conditions of Theorem~\ref{thm-area} are fulfilled for the set of all transient and final states.% (see Section~\ref{sec-prop-one-counter-unbounded}).

%the successors of either $\As{t}$ or $\Bs{t}$ are required  

%\noindent
% (C) If $\Ins_j \equiv \Halt$, i.e., $j = m{+}1$, then
% \begin{eqnarray*}
%     \Step_{i,\ell,x} & \equiv & \bZero \wedge \Hsuc_{i,\ell,x}
% \end{eqnarray*}
% where 
% \begin{eqnarray*}
%     \Hsuc_{i,\ell,a} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)} \vee \Ex{h,b,S^2(r_i)} \vee
%                              \Ex{h,c,S^2(r_i)}\big)\\  
%     \Hsuc_{i,\ell,b} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)} \vee \Ex{h,b,S^2(r_i),\ell_u} \vee
%                              \Ex{h,c,S^2(r_i)}\\
%     && \hspace*{5ex} \vee \Ex{h,c,S^2(r_i),e}\big) \ \wedge \ \opx_{=1{-}q} \Ex{h,c,S^2(r_i),e} 
% \end{eqnarray*}
% Recall that the counter is zero when $\M$ reaches $\Halt$ (see Section~\ref{sec-Minsky}). 

% \tikzstyle{state}=[draw,thick,minimum width=12mm,minimum height=12mm,rounded corners,text centered]
% \begin{figure*}[t]\centering
% \begin{tikzpicture}[x=1.7cm, y=1.7cm,scale=0.9,font=\small]
% \node (t) at (0,0) [state, draw=none] {\LARGE$\bullet$};
% \node [below of = t,node distance=3ex] (pt) {$\Ex{b,r_i,\ell_j}$};
% \node [above of = t, node distance=2ex] (lt) {$t$};
% % \begin{scope}[shift={(8.5,-1)}]
% %     \node (t1) at (0,0) [state] {};
% %     \node [below of = t1] (pt1) {$\Ex{h,b,S^2(r_i)}$};
% %     \node (t2) at (2,0) [state] {};
% %     \node [below of = t2] (pt2) {$\Ex{h,c,S^2(r_i)}$};
% % \end{scope}
% \begin{scope}[shift={(8,0.5)}]
%     \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
%     \node [above of = u, node distance=2ex] (lu) {$u_1\hspace{5.5ex}u_k$};
%     \node [below of = u] (pu) {$\Ex{a,S(r_i)}$};
%     \node (z1) at (-5.2,-2.7) [state] {};
%     \node [below of = z1] (pz1) {$\Ex{a,S^2(r_i)}$};
%     \node (z2) at (-4,-2.7) [state] {};
%     \node [below of = z2] (pz2) {$\Ex{h,b,S^3(r_i)}$};
%     \node (z3) at (-2.8,-2.7) [state] {};
%     \node [below of = z3] (pz3) {$\Ex{h,c,S^3(r_i)}$};
%     \node (zk1) at (-.7,-2.7) [state] {};
%     \node [below of = zk1] (pzk1) {$\Ex{a,S^2(r_i))}$};
%     \node (zk2) at (0.5,-2.7) [state] {};
%     \node [below of = zk2] (pzk2) {$\Ex{h,b,S^3(r_i)}$};
%     \node (zk3) at (1.7,-2.7) [state] {};
%     \node [below of = zk3] (pzk3) {$\Ex{h,c,S^3(r_i)}$};
%     \draw [thick, dotted] ($(z3) +(.7,0)$)  -- ($(zk1) +(-.7,0)$);
%     \draw[-stealth,rounded corners,thick] (t.center) -| node[left, near end] {$\vec{v}[t]_1$} (u);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u_k]_1$} (zk1);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u_k]_2$} (zk2);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {} (zk3);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u_1]_1$} (z1);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u_1]_2$} (z2);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);
% \end{scope}
% \begin{scope}[shift={(8,-3)}]
%     \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
%     \node [above of = u, node distance=2ex] (lu) {$\widehat{u}_1\hspace{5.8ex}\widehat{u}_{\widehat{k}}$};
%     \node [below of = u] (pu) {$\Ex{b,S^2(r_i),\ell_u}$};
%     \node (z1) at (-6.4,-2.7) [state] {};
%     \node [below of = z1] (pz1) {$a,S^3(r_i)$};
%     \node (z2) at (-5.2,-2.7) [state] {};
%     \node [below of = z2] (pz2) {$b,S^4(r_i)$};
%     \node (z3) at (-4,-2.7) [state] {};
%     \node [below of = z3] (pz3) {$c,S^4(r_i),\neg e$};
%     \node (z4) at (-2.8,-2.7) [state] {};
%     \node [below of = z4] (pz4) {$c,S^4(r_i),e$};
% %
%     \node (zk1) at (-.7,-2.7) [state] {};
%     \node [below of = zk1] (pzk1) {$a,S^3(r_i)$};
%     \node (zk2) at (0.5,-2.7) [state] {};
%     \node [below of = zk2] (pzk2) {$b,S^4(r_i)$};
%     \node (zk3) at (1.7,-2.7) [state] {};
%     \node [below of = zk3] (pzk3) {$c,S^4(r_i),\neg e$};
%     \node (zk4) at (2.9,-2.7) [state] {};
%     \node [below of = zk4] (pzk3) {$c,S^4(r_i),e$};
% %    
%     \draw [thick, dotted] ($(z4) +(.7,0)$)  -- ($(zk1) +(-.7,0)$);
%     \draw[-stealth,rounded corners,thick] (t.center) -- ++(.6,0) -- ++(0,-3.5) -| node[left, near end] {$\vec{v}[t]_2$} (u);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[\widehat{u}_{\widehat{k}}]_1$} (zk1);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[\widehat{u}_{\widehat{k}}]_2$} (zk2);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {} (zk3);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$1{-}q$} (zk4);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[\widehat{u}_1]_1$} (z1);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[\widehat{u}_1]_2$} (z2);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$1{-}q$} (z4);
% \end{scope}
% \begin{scope}[shift={(8,-6.3)}]
%     \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
%     \node [above of = u, node distance=2ex] (lu) {$u'_1\hspace{5.8ex}u'_{k'}$};
%     \node [below of = u] (pu) {$\Ex{c,S^2(r_i)}$};
%     \node (z1) at (-6.4,-2.7) [state] {};
%     \node [below of = z1] (pz1) {$\Ex{a,S^3(r_i)}$};
%     \node (z2) at (-5.2,-2.7) [state] {};
%     \node [below of = z2] (pz2) {$\Ex{h,b,S^4(r_i)}$};
%     \node (z3) at (-4,-2.7) [state] {};
%     \node [below of = z3] (pz3) {$\Ex{h,c,S^4(r_i)}$};
%     \node (z4) at (-2.8,-2.7) [state] {};
%     \node [below of = z4] (pz4) {$\Ex{h,c,S^4(r_i),d}$};
% %
%     \node (zk1) at (-.7,-2.7) [state] {};
%     \node [below of = zk1] (pzk1) {$\Ex{a,S^3(r_i))}$};
%     \node (zk2) at (0.5,-2.7) [state] {};
%     \node [below of = zk2] (pzk2) {$\Ex{h,b,S^4(r_i)}$};
%     \node (zk3) at (1.7,-2.7) [state] {};
%     \node [below of = zk3] (pzk3) {$\Ex{h,c,S^4(r_i)}$};
%     \node (zk4) at (2.9,-2.7) [state] {};
%     \node [below of = zk4] (pzk3) {$\Ex{h,c,S^4(r_i),d}$};
% %    
%     \draw [thick, dotted] ($(z4) +(.7,0)$)  -- ($(zk1) +(-.7,0)$);
%     \draw[-stealth,rounded corners,thick] (t.center) -- ++(.6,0) -- ++(0,-7) -|  (u);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u'_{k'}]_1$} (zk1);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u'_{k'}]_2$} (zk2);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {} (zk3);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -|  (zk4);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u'_1]_1$} (z1);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u'_1]_2$} (z2);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -|  (z4);
% \end{scope}
% \begin{scope}[shift={(8,-9.5)}]
%     \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
%     \node [above of = u, node distance=2ex] (lu) {$\ \ u''_1\hspace{5ex}u''_{k''}$};
%     \node [below of = u] (pu) {$\Ex{c,S^2(r_i),e}$};
%     \node (z1) at (-6.4,-2.7) [state] {};
%     \node [below of = z1] (pz1) {$\Ex{a,S^3(r_i)}$};
%     \node (z2) at (-5.2,-2.7) [state] {};
%     \node [below of = z2] (pz2) {$\Ex{h,b,S^4(r_i)}$};
%     \node (z3) at (-4,-2.7) [state] {};
%     \node [below of = z3] (pz3) {$\Ex{h,c,S^4(r_i)}$};
%     \node (z4) at (-2.8,-2.7) [state] {};
%     \node [below of = z4] (pz4) {$\Ex{h,c,S^4(r_i),d}$};
% %
%     \node (zk1) at (-.7,-2.7) [state] {};
%     \node [below of = zk1] (pzk1) {$\Ex{a,S^3(r_i))}$};
%     \node (zk2) at (0.5,-2.7) [state] {};
%     \node [below of = zk2] (pzk2) {$\Ex{h,b,S^4(r_i)}$};
%     \node (zk3) at (1.7,-2.7) [state] {};
%     \node [below of = zk3] (pzk3) {$\Ex{h,c,S^4(r_i)}$};
%     \node (zk4) at (2.9,-2.7) [state] {};
%     \node [below of = zk4] (pzk3) {$\Ex{h,c,S^4(r_i),d}$};
% %    
%     \draw [thick, dotted] ($(z4) +(.7,0)$)  -- ($(zk1) +(-.7,0)$);
%     \draw[-stealth,rounded corners,thick] (t.center) -- ++(.6,0) -- ++(0,-10.2) -| node[left, near end] {$1-q$}  (u);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u''_{k''}]_1$} (zk1);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {$\vec{v}[u''_{k''}]_2$} (zk2);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -| node[left, near end] {} (zk3);
%     \draw[-stealth,rounded corners,thick] ([xshift=4ex]u.center) -|  (zk4);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u''_1]_1$} (z1);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[u''_1]_2$} (z2);
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
%     \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -|  (z4);
% \end{scope}

% \end{tikzpicture}
% \caption{The structure of transient states satisfying $\Ex{b,r_i,\ell_j}$ where $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$}
% \label{fig-transient-oc}
% \end{figure*}

\tikzstyle{state}=[draw,thick,minimum width=12mm,minimum height=12mm,rounded corners,text centered]
\begin{figure*}[t]\centering
\begin{tikzpicture}[x=1.8cm, y=1.7cm,scale=0.80,font=\small]
\node (t) at (-1,0) [state, draw=none] {\LARGE$\bullet$};
\node [above of = t,node distance=3ex] (pt) {$\Ex{x,r_i,\ell_j}$};
\node [left of = t, node distance=2ex] (lt) {$t$};
% \begin{scope}[shift={(8.5,-1)}]
%     \node (t1) at (0,0) [state] {};
%     \node [below of = t1] (pt1) {$\Ex{h,b,S^2(r_i)}$};
%     \node (t2) at (2,0) [state] {};
%     \node [below of = t2] (pt2) {$\Ex{h,c,S^2(r_i)}$};
% \end{scope}
\begin{scope}[shift={(6,0.5)}]
    \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
    \node [above of = u, node distance=2.5ex] (lu) {$\As{t}$};
    \node [below of = u, xshift=-4ex, node distance=2ex] (luu) {$t_a'$};
    \node [below of = u, node distance=6.5ex] (pu) {$\Ex{a,S(r_i)}$};
    \node (z1) at (-5.2,-2.7) [state] {};
    \node [below of = z1] (pz1) {$a,S^2(r_i)$};
    \node (z2) at (-4,-2.7) [state] {};
    \node [below of = z2] (pz2) {$\Ex{h,b,S^3(r_i)}$};
    \node (z3) at (-2.8,-2.7) [state] {};
    \node [below of = z3] (pz3) {$\Ex{h,c,S^3(r_i)}$};
 %
    \draw[-stealth,rounded corners,thick] (t.center) -| node[left, near end] {$\vec{v}[t]_1$} (u);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_a']_1$} (z1);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_a']_2$} (z2);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);
\end{scope}
\begin{scope}[shift={(12,0.5)}]
    \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
    \node [above of = u, node distance=2.5ex] (lu) {$\Bs{t}$};
    \node [below of = u, xshift=-3.5ex, node distance=2ex] (luu) {$t_b'$};
    \node [below of = u, node distance=6.5ex] (pu) {$\Ex{b,S^2(r_i),\ell'}$};
    \node (z1) at (-6.4,-2.7) [state] {};
    \node [below of = z1] (pz1) {$a,S^3(r_i)$};
    \node (z2) at (-5.2,-2.7) [state] {};
    \node [below of = z2] (pz2) {$b,S^4(r_i)$};
    \node (z3) at (-4,-2.7) [state] {};
    \node [below of = z3] (pz3) {$c,S^4(r_i),\neg e$};
    \node (z4) at (-2.8,-2.7) [state] {};
    \node [below of = z4] (pz4) {$c,S^4(r_i),e$};
%    
    \draw[-stealth,rounded corners,thick] (t.center) -| node[left, near end] {$\vec{v}[t]_2$} (u);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_b']_1$} (z1);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_b']_2$} (z2);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$1{-}q$} (z4);
\end{scope}
\begin{scope}[shift={(6,-3)}]
    \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
    \node [above of = u, node distance=2ex] (lu) {};
    \node [below of = u, xshift=-3.5ex, node distance=2ex] (luu) {$t_c'$};
    \node [below of = u, node distance=6.5ex] (pu) {$\Ex{c,S^2(r_i)}$};
    \node (z1) at (-6.4,-2.7) [state] {};
    \node [below of = z1] (pz1) {$\Ex{a,S^3(r_i)}$};
    \node (z2) at (-5.2,-2.7) [state] {};
    \node [below of = z2] (pz2) {$\Ex{h,b,S^4(r_i)}$};
    \node (z3) at (-4,-2.7) [state] {};
    \node [below of = z3] (pz3) {$\Ex{h,c,S^4(r_i)}$};
    \node (z4) at (-2.8,-2.7) [state] {};
    \node [below of = z4] (pz4) {$\Ex{h,c,S^4(r_i),d}$};
%
    \draw[-stealth,rounded corners,thick] (t.center) -- ++(.6,0) -- ++(0,-3.5) -|  (u);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_c']_1$} (z1);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_c']_2$} (z2);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -|  (z4);
\end{scope}
\begin{scope}[shift={(12,-3)}]
    \node (u) at (-2,-1.5) [state] {\LARGE$\bullet\ \cdots \ \bullet$};
    \node [above of = u, node distance=2ex] (lu) {};
    \node [below of = u, xshift=-3ex, node distance=2ex] (luu) {$t_c''$};
    \node [below of = u, node distance=6.5ex] (pu) {$\Ex{c,S^2(r_i),e}$};
    \node (z1) at (-6.4,-2.7) [state] {};
    \node [below of = z1] (pz1) {$\Ex{a,S^3(r_i)}$};
    \node (z2) at (-5.2,-2.7) [state] {};
    \node [below of = z2] (pz2) {$\Ex{h,b,S^4(r_i)}$};
    \node (z3) at (-4,-2.7) [state] {};
    \node [below of = z3] (pz3) {$\Ex{h,c,S^4(r_i)}$};
    \node (z4) at (-2.8,-2.7) [state] {};
    \node [below of = z4] (pz4) {$\Ex{h,c,S^4(r_i),d}$};
%    
    \draw[-stealth,rounded corners,thick] (t.center) -- ++(.6,0) -- ++(0,-3.5) -| node[left, near end] {$1-q$}  (u);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_c'']_1$} (z1);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {$\vec{v}[t_c'']_2$} (z2);
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -| node[left, near end] {} (z3);   
    \draw[-stealth,rounded corners,thick] ([xshift=-4ex]u.center) -|  (z4);
\end{scope}

\end{tikzpicture}
\caption{The structure of transient states satisfying $\Ex{x,r_i,\ell_j}$ where $x \in \{a,b\}$ and $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$}
\label{fig-transient-oc}
\end{figure*}


\subsection{A Proof of Theorem~\ref{thm-one-counter}}

Let $\M \ \equiv\ 1: \Ins_1; \ \cdots  \ m: \Ins_m$ be a non-deterministic one-counter Minsky machine, and let $\psi$ be the formula constructed for $\M$ in Section~\ref{sec-one-counter-psi}. The two claims of Theorem~\ref{thm-one-counter} are proven separately in the following subsections.

% \begin{proposition}
% \label{prop-one-counter-unbounded}
%     Let $M =(S,P,v)$ be a finite-state model of $\psi$. Then for every reachable configuration $(j,n)$ of $\M$, there  exists a state $t \in S$ such that $t \models \ell_j$ and $\vec{v}[t] = \sigma^n(\vec{\kappa})$.
% \end{proposition}

% \begin{proposition}
% \label{prop-one-counter-bounded}   
%     If $\M$ is bounded, then $\psi$ has a finite-state model.
% \end{proposition}

% Note that Proposition~\ref{prop-one-counter-unbounded} implies that if $\M$ is not bounded, then the formula $\psi$ does not have a finite-state model. 

\subsubsection{A Proof of Theorem~\ref{thm-one-counter}~(A)}
\label{sec-prop-one-counter-unbounded}

Let $M =(S,P,v)$ be Markov chain and $s \in S$ such that $s \models \psi$.  Let $T$ be the set of all transient states and all final states of $M$. One can easily verify that the conditions of Theorem~\ref{thm-area} are satisfied for $T$ by inspecting the structure of transient states similarly as in Section~\ref{sec-proof-main-param} (in particular, the formula $\bEq_i$ still implies Equalities~\eqref{eq-convex-one} and~\eqref{eq-convex-two}). Thus, by applying Theorem~\ref{thm-area}, we obtain 
\begin{itemize}
    \item[I.] For every $t \in T$, we have that $\vec{v}[t] \in \Area(\vec{\kappa})$.
    \item[II.] For every $t \in T$ where $\vec{v}[t] \neq \vec{\kappa}$ and every $t' \in \As{t}$, we have that $\vec{v}[t']  = \tau(\vec{v}[t])$.
\end{itemize}

We show that $s$ simulates $\M$. Since $s \models \Init$, we have that $s$~represents the configuration $(1,0)$. Let $t$ be a state reachable from $s$ such that $t$ 
% . Then $t$ satisfies exactly one the formulae $\bFin$, $\bFree$, $\bTrans$, $\CTrans$, and $\LTrans$. It follows directly from the construction of $\psi$ that if $t \not\models \LTrans$, then $t \models \opg_{=1} \bigwedge_{i=1}^m \neg\ell_i$. Now, suppose that $t$ 
represents a configuration $(j,n)$ of~$\M$, i.e., $t \models \ell_j$ and $\vec{v}[t] = \sigma^n(\vec{\kappa})$. Then $t \models \LTrans$ and hence also $t \models \Step_{i,\ell_j}$. We distinguish two cases.
\smallskip

\noindent
(A) $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } L \textit{ else dec } c; \textit{ goto } L'$.\quad Then, 
\begin{eqnarray*}
    \Step_{i,\ell} & \equiv & \hspace*{2ex} \left(\bZero \Rightarrow (\Zsuc_{i,\ell} \wedge \opx_{=1} (b \Rightarrow \bZero))\right)\\
    && \wedge \left( \neg\bZero \Rightarrow (\Psuc_{i,\ell} \wedge \bInterval \wedge \bEq_i ) \right)
\end{eqnarray*}
and there are two subcases.
\begin{itemize}
    \item $n=0$.  Since $\vec{v}[t] = \sigma^n(\vec{\kappa})$, we obtain $t \models \bZero$. Hence, $t \models \Zsuc_{i,\ell} \wedge \opx_{=1} (b \Rightarrow \bZero)$. This implies that every $t' \in \Bs{t}$ satisfies $t' \models \Ex{b,S^2(r_i),\ell'} \wedge \bZero$ for some $\ell' \in L$. Hence, $t'$ represents a successor configuration of $(j,0)$. 
    Since $\vec{v}[t]_2 = \vec{\kappa}_2 > 0$, we have $\Bs{t} \neq \emptyset$, and hence at least one such $t'$ exists. Furthermore, all states of $\As{t} \cup \Cs{t}$ are free and hence they satisfy the formula $\opg_{=1} \bigwedge_{i=1}^m \neg\ell_i$.
    \item $n > 0$. Since $\vec{v}[t] = \sigma^n(\vec{\kappa})$, we obtain $t \models \neg\bZero$ and hence $t \models \Psuc_{i,\ell} \wedge \bInterval \wedge \bEq_i$. The formula $\Psuc_{i,\ell}$ ensures that every $t' \in \As{t}$  satisfies $t' \models \Ex{a,S(r_i),\ell'}$ for some \mbox{$\ell' \in L'$}. Furthermore, we have that $\vec{v}[t'] = \tau(\sigma^n(\vec{\kappa})) =  \sigma^{n-1}(\vec{\kappa})$ by Observation~II.~above. Hence, $t'$ represents a successor configuration of $(j,n)$. Since $\vec{v}[t]_1 = \sigma^n(\vec{\kappa})_1 > 0$, at least one such $t'$ must exist. Note that all states of $\Bs{t} \cup \Cs{t}$ satisfy the formula $\opg_{=1} \bigwedge_{i=1}^m \neg\ell_i$.
\end{itemize}

\noindent
(B) $\Ins_j \equiv \textit{inc } c; \textit{ goto } L$.\quad Then, %Let us first consider the case $x = b$, i.e., 
\begin{eqnarray*}
    \Step_{i,\ell} & \equiv & 
    \hspace*{2ex} (\bZero \Rightarrow \IZsuc_{i,\ell})\\
    && \wedge \ (\neg\bZero \Rightarrow (\IPsuc_{i,\ell} \wedge \bInterval \wedge \bEq_i)\\
    && \wedge \ \opf^2_{=1{-}q} (a\wedge S^3(r_i))\\
    && \wedge \ \opf^2_{=\gamma} \big((b \wedge S^4(r_i) ) \vee d\big)\\
    && \wedge \ \opf^2_{=\gamma} \big((c\wedge S^4(r_i) \wedge e) \vee d \big)
\end{eqnarray*}
% where
% \begin{eqnarray*}
%     % \IZsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)} \vee \Ex{b,S^2(r_i),\ell_u} \vee
%     % \Ex{c,S^2(r_i)}\\
%     % && \hspace*{5ex}  \vee \Ex{c,S^2(r_i),e} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}\\
%     % \IPsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{a,S(r_i)} \vee \Ex{b,S^2(r_i),\ell_u} \vee
%     % \Ex{c,S^2(r_i)}\\
%     % && \hspace*{5ex}  \vee \Ex{c,S^2(r_i),e} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}
%     \IZsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{h,a,S(r_i)}  \vee
%     \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\
%     && \hspace*{5ex}  \vee \bigvee_{\ell' \in L} \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}\\
%     \IPsuc_{i,\ell} & \equiv & \opx_{=1} \big(\Ex{a,S(r_i)}  \vee
%     \Ex{c,S^2(r_i)} \vee \Ex{c,S^2(r_i),e}\\
%     && \hspace*{5ex}  \vee \bigvee_{\ell' \in L} \Ex{b,S^2(r_i),\ell'} \big) \ \wedge \ \opx_{=1{-}q} \Ex{c,S^2(r_i),e}
% \end{eqnarray*}   
 
The structure of immediate successors of $t$ enforced by this formula is shown in Fig.~\ref{fig-transient-oc}. The formulae $\IZsuc_{i,\ell}$ and $\IPsuc_{i,\ell}$ ensure that for every $t' \in \Bs{t}$, we have that $t' \models \Ex{b,S^2(r_i),\ell'}$ where $\ell' \in L$. 
Observe that $\Bs{t} \neq \emptyset$ and all states of $\As{t} \cup \Cs{t}$ satisfy the formula $\opg_{=1} \bigwedge_{i=1}^m \neg\ell_i$. Hence, it remains to show that $\vec{v}[t'] = \sigma(\vec{v}[t])$ for all $t' \in \Bs{t}$. We prove a stronger result saying that
$\vec{v}[t'] = \sigma(\vec{v}[t])$ for all $t' \in \Bs{t} \cup \Cs{t}$.

Due to Observation~I above and Lemma~\ref{lem-gproperties}.A, it suffices to prove that $\sigma(\vec{v}[t])$ is a positive convex combination of the vectors in $\{\vec{v}[t'] \mid t' \in \Bs{t} \cup \Cs{t}\}$. For a path formula $\Phi$, we use $R[\Phi]$ to denote the set of all $w \in \run(t)$ such that $w \models \Phi$.

Since $t \models \opf^2_{=1{-}q} (a\wedge S^3(r_i))$, we have $\m_t(R[\opf^2(a\wedge S^3(r_i))]) = 1{-}q$.
By inspecting the structure of immediate successors of~$t$ (see Fig.~\ref{fig-transient-oc}), we obtain
\begin{equation}
   1{-}q \ = \ \m_t(R[\opf^2(a\wedge S^3(r_i))]) \ = \ \sum_{t' \in \Bs{t} \cup \Cs{t}} P(t,t') \cdot \vec{v}[t']_1\,.
\label{eq-sigma-one}   
\end{equation}
Observe that $\sum_{t' \in \Bs{t} \cup \Cs{t}} P(t,t') = 1 {-} \vec{v}[t]_1$. Hence, \eqref{eq-sigma-one} implies
\begin{equation}
   \frac{1{-}q}{1 {-} \vec{v}[t]_1} \ =  \ \sum_{t' \in \Bs{t} \cup \Cs{t}} \frac{P(t,t')}{1 {-} \vec{v}[t]_1} \cdot \vec{v}[t']_1 \,.
\label{eq-sigma-first}
\end{equation}
Note that the left-hand side of~\eqref{eq-sigma-first} is equal to $\sigma(\vec{v}[t])_1$. 

Furhermore, $t \models \opf^2_{=\gamma} \big((b \wedge S^4(r_i) ) \vee d\big)$. By inspecting the structure of immediate successors of~$t$ (see Fig.~\ref{fig-transient-oc}), we obtain\footnote{Here, by writing $C = A \uplus B$ we mean that $C = A \cup B$ and $A \cap B = \emptyset$.}
\begin{eqnarray}
   \gamma & = & \m_t(R[\opf^2((b \wedge S^4(r_i) ) \vee d)]) \nonumber \\
       & = & \m_t(R[\opf^2(b \wedge S^4(r_i))] \uplus R[\opf^2(d)]) \nonumber \\
       & = & \m_t(R[\opf^2(b \wedge S^4(r_i))]) \  \ + \ \  \m_t(R[\opf^2(d)]) \nonumber \\
       & = & \sum_{t' \in \Bs{t} \cup \Cs{t}} P(t,t') \cdot \vec{v}[t']_2 \ \ + \ \ \m_t(R[\opf^2(d)])
\label{eq-sigma-F1}
\end{eqnarray}

Similarly, $t \models \opf^2_{=\gamma} \big((c\wedge S^4(r_i) \wedge e) \vee d \big)$ implies
\begin{eqnarray}
    \gamma & = & \m_t(R[\opf^2((c\wedge S^4(r_i) \wedge e) \vee d)]) \nonumber \\
        & = & \m_t(R[\opf^2(c\wedge S^4(r_i) \wedge e)] \uplus R[\opf^2(d)]) \nonumber \\
        & = & \m_t(R[\opf^2(c \wedge S^4(r_i) \wedge e)]) \  \ + \ \  \m_t(R[\opf^2(d)]) \nonumber \\
        & = & \sum_{t' \in \Bs{t}} P(t,t') \cdot (1{-}q) \ \ + \ \ \m_t(R[\opf^2(d)]) \nonumber \\
        & = & \vec{v}[t]_2 \cdot (1{-}q) \ \ + \ \ \m_t(R[\opf^2(d)])
 \label{eq-sigma-F2}
\end{eqnarray}

Since the right-hand sides of \eqref{eq-sigma-F1} and \eqref{eq-sigma-F2} are equal, we have that
\begin{equation*}
    \vec{v}[t]_2 \cdot (1{-}q) = \sum_{t' \in \Bs{t} \cup \Cs{t}} P(t,t') \cdot \vec{v}[t']_2
\end{equation*}
Hence,
\begin{equation}
    \frac{\vec{v}[t]_2 \cdot (1{-}q)}{1 {-} \vec{v}[t]_1} = \sum_{t' \in \Bs{t} \cup \Cs{t}} \frac{P(t,t')}{1 {-} \vec{v}[t]_1} \cdot \vec{v}[t']_2
\label{eq-sigma-second}
\end{equation}
Observe that the left-hand side of~\eqref{eq-sigma-second} is equal to $\sigma(\vec{v}[t])_2$. By combining~\eqref{eq-sigma-first} and~\eqref{eq-sigma-second}, we finally obtain
\[
    \sigma(\vec{v}[t]) \ = \ \sum_{t' \in \Bs{t} \cup \Cs{t}} \frac{P(t,t')}{1 {-} \vec{v}[t]_1} \cdot \vec{v}[t']\,.
\] 

%The case when $x = a$ is similar and does not require any new insights. 
\subsubsection{A Proof of Theorem~\ref{thm-one-counter}~(B)}
\label{sec-proof-prop-one-counter-bounded}

For the rest of this proof, we fix a computation $\omega = C_0,C_1,\ldots$ of $\M$. Furthermore, if $\omega$ is periodic, we fix $\alpha,\beta$ such that $\alpha < \beta$ and the infinite sequences $C_{\alpha-1},C_{\alpha},C_{\alpha+1},\ldots$ and $C_{\beta-1},C_{\beta},C_{\beta+1},\ldots$ are the same. If $\omega$ is not periodic, we put $\beta = \infty$ and leave $\alpha$ undefined.

Observe that if $\omega$ is periodic, then our choice of $\alpha$ and $\beta$ ensures that the infinite sequences $C_{\alpha},C_{\alpha+1},\ldots$ and $C_\beta,C_{\beta+1},\ldots$ are also the same, and the compuational steps $C_{\alpha-1} \mapsto C_{\alpha}$ and  $C_{\beta-1} \mapsto C_{\beta}$ are generated by the same instruction of $\M$. As we shall see, this ensures that $C_\alpha$ and $C_\beta$ are represented by the same state in the constructed model of $\psi$. 

We show that there exist a Markov chain $M = (S,P,v)$ and a state $s \in S$ such that $s \models \psi$ and $s$ covers $\omega$. Furthermore, if $\beta < \infty$, then $S$ is finite.

Every state of $S$ is a triple of the form $[\iota,\calL,n]$ where $\iota$ is an index ranging over $\{i \in \N \mid 0\leq i < \beta\} \cup \{\star\}$, $\calL \subseteq \A$ is the set of atomic propositions satisfied in the state, and $n \in \N \cup \{\star\}$ is a counter value. The $\star$ symbol is used when the index or the counter value (or both) are not relevant. 

The Markov chain $M$ is the least Markov chain $M'$ such that $s \equiv [0,\{a,r_0,\ell_1\},0]$ is a state of $M'$, and if $t$ is a state of $M'$ then $M'$ contains all immediate successors of $t$ defined by the following rules:
\smallskip

\noindent
\textbf{Rule I.} If $t = [k,\{x,r_i,\ell_j\},n]$ where $x \in \{a,b\}$, $C_{k} = (j,n)$, and $k < \beta$, then the immediate successors of $t$ are determined as follows. First, let $k'$ be either $\alpha$ or $k+1$ depending on whether $k=\beta - 1$ or $k < \beta -1$, respectively.
Furthermore, let $C_{k'} = (j',n')$, and let $t'$ be either $[k',\{a,S(r_i),\ell_{j'}\},n']$ or $[k',\{b,S^2(r_i),\ell_{j'}\},n']$, depending on whether $n' = n-1$ or $n' \geq n$, respectively. 

Now we distinguish four possibilities (the cases when $\Ins_j$ is a Type~II and Type~I instruction are covered by~(A)--(B) and (C)--(D), respectively. In each case, we distinguish between zero and positive counter values represented by the~$n$).
\smallskip

\noindent
\textbf{(A)} $n' = n = 0$. Then,
\begin{eqnarray*}
    P(t,[\star,\{h,a,S(r_i)\},\star]) & = & \vec{\kappa}_1,\\
    P(t,t') & = & \vec{\kappa}_2,\\
    P(t,[\star,\{h,c,S^2(r_i),e\},\star]) & = & 1 {-} q,\\
    P(t,[\star,\{h,c,S^2(r_i)\},\star]) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 \,.
\end{eqnarray*}

\noindent
\textbf{(B)} $n' = n-1$. We put
\begin{eqnarray*}
    P(t,t') & = & \sigma^n(\vec{\kappa})_1,\\
    P(t,[\star,\{h,b,S^2(r_i)\},\star]) & = & \sigma^n(\vec{\kappa})_2,\\ 
    P(t,[\star,\{h,c,S^2(r_i),e\},\star]) & = & 1 {-} q,\\
    P(t,[\star,\{h,c,S^2(r_i)\},\star]) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 \,.
\end{eqnarray*}

\noindent
\textbf{(C)} $n' = 1$ and $n = 0$. Then,
\begin{eqnarray*}
    P(t,[\star,\{h,a,S(r_i)\},\star]) & = & \vec{\kappa}_1,\\
    P(t,t') & = & \vec{\kappa}_2,\\
    P(t,[\star,\{c,S^2(r_i),e\},1]) & = & 1 {-} q,\\
    P(t,[\star,\{c,S^2(r_i)\},1]) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
\end{eqnarray*}

\noindent
\textbf{(D)} $n' = n+1$ and $n > 0$. Then,
\begin{eqnarray*}
    P(t,[\star,\{a,S(r_i)\},n{-}1]) & = & \sigma^n(\vec{\kappa})_1,\\
    P(t,t') & = & \sigma^n(\vec{\kappa})_2,\\
    P(t,[\star,\{c,S^2(r_i),e\},n{+}1]) & = & 1{-}q,\\
    P(t,[\star,\{c,S^2(r_i)\},n{+}1]) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
\end{eqnarray*}

\noindent
\textbf{Rule II.} If $t = [\star,\{a,r_i\},n]$ where $n \geq 0$, we have the following:
\begin{eqnarray*}
    \mbox{if $n = 0$, then}\hspace*{1.2em} P(t,[\star,\{h,a,S(r_i)\},\star]) & = & 
       \sigma^n(\vec{\kappa})_1 = \vec{\kappa}_1,\\
    \mbox{if $n > 0$, then}\hspace*{1em} P(t,[\star,\{a,S(r_i)\},n{-}1]) & = & \sigma^n(\vec{\kappa})_1,\\
    P(t,[\star,\{h,b,S^2(r_i)\},\star]) & = & \sigma^n(\vec{\kappa})_2,\\
    P(t,[\star,\{h,c,S^2(r_i)\},\star]) & = & 1 {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
\end{eqnarray*}

\noindent
\textbf{Rule III.} If $t = [\star,\calL,n]$ where $n>0$ and $\calL$ is $\{c,r_i\}$ or $\{c,r_i,e\}$, then
\begin{eqnarray*}
    P(t,[\star,\{a,S(r_i)\},n{-}1))         & = & \sigma^n(\vec{\kappa})_1,\\
    P(t,[\star,\{h,b,S^2(r_i)\},\star)      & = & \sigma^n(\vec{\kappa})_2,\\
    P(t,[\star,\{h,c,S^2(r_i),d\},\star)    & = & p_n,\\
    P(t,[\star,\{h,c,S^2(r_i)\},\star)      & = & 1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2 - p_n
\end{eqnarray*}
where 
\[
     p_n = \frac{\gamma - (1{-}q) \sigma^{n-1}(\vec{\kappa})_2}{1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2}    
\]
% Note that $S$ does \emph{not} contain any state of the form $[\star,\calL,0]$ where $\calL$ is $\{c,r_i\}$ or $\{c,r_i,e\}$. Also 
Note that $0 < p_n < 1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2$ due to the constraints imposed on $\gamma$ and $\vec{\kappa}$ at the beginning of Section~\ref{sec-counter}. More precisely, the constraint $\gamma > (1{-}q) \vec{\kappa}_2$ ensures that $p_n > 0$, and the constraint $\gamma < \frac{3}{4}q - \frac{5}{4}q + \frac{1}{2}q^2$ ensures that 
$2p_n < 1 - (2 (q{-}\frac{1}{2})+ (1{-}q))$ (recall that $\vec{\kappa}_1 + \vec{\kappa}_1 < q - \frac{1}{2}$ and $\sigma^{m}(\vec{\kappa})$ is strictly less than $\vec{\kappa}$ in both components for every $m \geq 0$). This is more than we need here; the constraints are chosen so that they also satisfy stronger requirements needed in the proof of Theorem~\ref{thm-two-counter}.
\smallskip

\noindent
\textbf{Rule IV.} If $t =[\star,\calL,\star]$, then $P(t,t) = 1$. 
\smallskip

Note that if $\omega$ is periodic, then $M$ has finitely many states. It is easy to check that $s \models \psi$ by verifying that every state of $M$ satisfies either $\bFin$, $\Transient$, or $\bFree$. In particular, every state of the form $[\iota,\{b,r_i,\ell_j\},n]$ where $\Ins_j$ is a Type~I instruction satisfies
$\opf^2_{=\gamma} \big((b \wedge S^4(r_i) ) \vee d\big)$ and
$\opf^2_{=\gamma} \big((c\wedge S^4(r_i) \wedge e) \vee d \big)$. This is where we need the constant $p_n$ of Rule~III. Clearly, $s$ covers the computation~$\omega$ (and no other computation).


% Suppose that $\M$ is bounded. We show that then $\psi$ has a finite-state model $M = (S,P,v)$, where every  $t \in S$ is a list of all atomic propositions of $\A$ that are satisfied in $t$, possibly extended with a single integer representing the current counter value. 

% The set $S$ and the transition function $P$ are constructed gradually as follows (note that $v(t)$ is determined implicitly by the list of atomic propositions occurring in $t$):

% \begin{itemize}
%     \item Initially, we put $S = \{(a,r_0,\ell_1,0)\}$ where the state $(a,r_0,\ell_1,0)$ is declared as \emph{unprocessed}.
%     \item As long as $S$ contains an unprocessed state $t$, we define the immediate successors of $t$ together with the value of the transition function, and change the status of $t$ to \emph{processed}. The immediate successors of $t$ that are missing in the current $S$ are automatically inserted into $S$ and declared as unprocessed.
% \end{itemize}

% Processing of $t$ depends on the form of $t$. We distinguish several cases (note that \textbf{(A)}--\textbf{(D)} cover all possibilities).
% \smallskip

% \noindent
% \textbf{(A)} $t \equiv [\iota, \{x,r_i,\ell_j\}, n)$ where $\iota < \beta$ and $x \in \{a,b\}$. There are two subcases.
% \smallskip

% \noindent
% (Aa) $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } u \textit{ else dec } c; \textit{ goto } u'$. If $n=0$, then 
% \begin{eqnarray*}
%     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
%     P(t,(b,S^2(r_i),\ell_u,0)) & = & \vec{\kappa}_2,\\
%     P(t,(h,c,S^2(r_i),e)) & = & 1 {-} q,\\
%     P(t,(h,c,S^2(r_i))) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% \end{eqnarray*}
% If $n > 0$, then
% \begin{eqnarray*}
%     P(t,(a,S(r_i),\ell_{u'},n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(h,b,S^2(r_i))) & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(h,c,S^2(r_i),e)) & = & 1 {-} q,\\
%     P(t,(h,c,S^2(r_i))) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
% \end{eqnarray*}

% \noindent
% (Ab) $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$. If $n = 0$, then 
% \begin{eqnarray*}
%     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
%     P(t,(b,S^2(r_i),\ell_u,1)) & = & \vec{\kappa}_2,\\
%     P(t,(c,S^2(r_i),e,1)) & = & 1 {-} q,\\
%     P(t,(c,S^2(r_i),1)) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% \end{eqnarray*}
% If $n > 0$, then
% \begin{eqnarray*}
%     P(t,(a,S(r_i),n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(b,S^2(r_i),\ell_u,n{+}1)) & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(c,S^2(r_i),e,n{+}1)) & = & 1{-}q,\\
%     P(t,(c,S^2(r_i),n{+}1)) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
% \end{eqnarray*}





% % \noindent
% % \textbf{(A)} $t \equiv (x,r_i,\ell_j,k)$, where $x \in \{a,b\}$. Then, there are two subcases.
% % \smallskip

% % \noindent
% % (Aa) $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } u \textit{ else dec } c; \textit{ goto } u'$. If $k=0$, then 
% % \begin{eqnarray*}
% %     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
% %     P(t,(b,S^2(r_i),\ell_u,0)) & = & \vec{\kappa}_2,\\
% %     P(t,(h,c,S^2(r_i))) & = & 1 {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% % \end{eqnarray*}
% % If $k > 0$, then
% % \begin{eqnarray*}
% %     P(t,(a,S(r_i),\ell_{u'},k{-}1)) & = & \sigma^k(\vec{\kappa})_1,\\
% %     P(t,(h,b,S^2(r_i))) & = & \sigma^k(\vec{\kappa})_2,\\
% %     P(t,(h,c,S^2(r_i))) & = & 1 {-} \sigma^k(\vec{\kappa})_1 {-} \sigma^k(\vec{\kappa})_2 
% % \end{eqnarray*}

% % \noindent
% % (Ab) $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$. If $k = 0$, then 
% % \begin{eqnarray*}
% %     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
% %     P(t,(b,S^2(r_i),\ell_u,1)) & = & \vec{\kappa}_2,\\
% %     P(t,(c,S^2(r_i),1)) & = & 1 {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% % \end{eqnarray*}
% % If $k > 0$, then
% % \begin{eqnarray*}
% %     P(t,(a,S(r_i),k{-}1)) & = & \sigma^k(\vec{\kappa})_1,\\
% %     P(t,(b,S^2(r_i),\ell_u,k{+}1)) & = & \sigma^k(\vec{\kappa})_2,\\
% %     P(t,(c,S^2(r_i),k{+}1)) & = & 1 {-} \sigma^k(\vec{\kappa})_1 {-} \sigma^k(\vec{\kappa})_2 
% % \end{eqnarray*}



% % \noindent
% % (Ac) $\Ins_j \equiv \Halt$, i.e., $j = m{+}1$. Then
% % \begin{eqnarray*}
% %     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
% %     P(t,(h,b,S^2(r_i))) & = & \vec{\kappa}_2,\\
% %     P(t,(h,c,S^2(r_i))) & = & 1 {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% % \end{eqnarray*}

% \noindent
% \textbf{(A)} $t \equiv (x,r_i,\ell_j,n)$ where $x \in \{a,b\}$. There are two subcases.
% \smallskip

% \noindent
% (Aa) $\Ins_j \equiv \textit{if } c{=}0 \textit{ then goto } u \textit{ else dec } c; \textit{ goto } u'$. If $n=0$, then 
% \begin{eqnarray*}
%     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
%     P(t,(b,S^2(r_i),\ell_u,0)) & = & \vec{\kappa}_2,\\
%     P(t,(h,c,S^2(r_i),e)) & = & 1 {-} q,\\
%     P(t,(h,c,S^2(r_i))) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% \end{eqnarray*}
% If $n > 0$, then
% \begin{eqnarray*}
%     P(t,(a,S(r_i),\ell_{u'},n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(h,b,S^2(r_i))) & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(h,c,S^2(r_i),e)) & = & 1 {-} q,\\
%     P(t,(h,c,S^2(r_i))) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
% \end{eqnarray*}

% \noindent
% (Ab) $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$. If $n = 0$, then 
% \begin{eqnarray*}
%     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
%     P(t,(b,S^2(r_i),\ell_u,1)) & = & \vec{\kappa}_2,\\
%     P(t,(c,S^2(r_i),e,1)) & = & 1 {-} q,\\
%     P(t,(c,S^2(r_i),1)) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% \end{eqnarray*}
% If $n > 0$, then
% \begin{eqnarray*}
%     P(t,(a,S(r_i),n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(b,S^2(r_i),\ell_u,n{+}1)) & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(c,S^2(r_i),e,n{+}1)) & = & 1{-}q,\\
%     P(t,(c,S^2(r_i),n{+}1)) & = & q {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
% \end{eqnarray*}

% % \noindent
% % (Bc) $\Ins_j \equiv \Halt$, i.e., $j = m{+}1$. Then
% % \begin{eqnarray*}
% %     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
% %     P(t,(h,b,S^2(r_i))) & = & \vec{\kappa}_2,\\
% %     P(t,(h,c,S^2(r_i),e)) & = & 1 {-} q,\\
% %     P(t,(h,c,S^2(r_i))) & = & q {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% % \end{eqnarray*}

% \noindent
% \textbf{(B)} $t \equiv (a,r_i,n)$. If $n = 0$, then
% \begin{eqnarray*}
%     P(t,(h,a,S(r_i))) & = & \vec{\kappa}_1,\\
%     P(t,(h,b,S^2(r_i))) & = & \vec{\kappa}_2,\\
%     P(t,(h,c,S^2(r_i))) & = & 1 {-} \vec{\kappa}_1 {-} \vec{\kappa}_2 
% \end{eqnarray*}
% If $n > 0$, then
% \begin{eqnarray*}
%     P(t,(a,S(r_i),n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(h,b,S^2(r_i)) & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(h,c,S^2(r_i)) & = & 1 {-} \sigma^n(\vec{\kappa})_1 {-} \sigma^n(\vec{\kappa})_2 
% \end{eqnarray*}

% \noindent 
% \textbf{(C)} $t \equiv (c,r_i,n)$ or $t \equiv (c,r_i,e,n)$. Then $n>0$, and we put
% \begin{eqnarray*}
%     P(t,(a,S(r_i),n{-}1)) & = & \sigma^n(\vec{\kappa})_1,\\
%     P(t,(h,b,S^2(r_i))    & = & \sigma^n(\vec{\kappa})_2,\\
%     P(t,(h,c,S^2(r_i),d)    & = & p_n,\\
%     P(t,(h,c,S^2(r_i))    & = & 1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2 - p_n
% \end{eqnarray*}
% where 
% \[
%      p_n = \frac{\gamma - (1{-}q) \sigma^{n-1}(\vec{\kappa})_2}{1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2}    
% \]
% Note that $0 < p_n < 1 - \sigma^n(\vec{\kappa})_1 - \sigma^n(\vec{\kappa})_2$ due to the constraints imposed on $\gamma$ and $\vec{\kappa}$ at the beginning of Section~\ref{sec-counter}. More precisely, the constraint $\gamma > (1{-}q) \vec{\kappa}_2$ ensures that $p_n > 0$, and the constraint $\gamma < \frac{3}{4}q - \frac{5}{4}q + \frac{1}{2}q^2$ ensures that 
% $2p_n < 1 - (2 (q{-}\frac{1}{2})+ (1{-}q))$ (recall that $\vec{\kappa}_1 + \vec{\kappa}_1 < q - \frac{1}{2}$ and $\sigma^{m}(\vec{\kappa})$ is strictly less than $\vec{\kappa}$ in both components for every $m \geq 0$). This is more than we need here; the constraints are chosen so that they also satisfy the stronger requirements needed in the proof of Proposition~\ref{prop-Minsky-bounded}.

% \smallskip

% \noindent 
% \textbf{(D)} $t$ contains $h$. Then $P(t,t) =1$.
% \smallskip

% Since $\M$ is bounded, the above construction terminates and produces a Markov chain where the number of states is proportional to the number of reachable configurations of $\M$. It is easy to check that $(a,r_0,\ell_1,0) \models \psi$ by verifying that every $t\in S$ satisfies either $\bFin$, $\Transient$, or $\bFree$ (this requires a routine inspection of the states reachable from $t$ in at most two steps). In particular, note that every state of the form $(b,r_i,\ell_j,k)$ where $\Ins_j \equiv \textit{inc } c; \textit{ goto } u$ satisfies
% $\opf^2_{=\gamma} \big((b \wedge S^4(r_i) ) \vee d\big)$ and
% $\opf^2_{=\gamma} \big((c\wedge S^4(r_i) \wedge e) \vee d \big)$. This is where we need the constant $p_n$ of $\textbf{(D)}$.

% It is worth noting that if $\M$ is unbounded, then the infinite-state Markov chain obtained as the least fixed point of the extension operator defined by the above rules is a model of $\psi$. 

==> fgnotes.tex <==
\section{Notes about $\opf,\opg$-fragment}

\subsection{Implementing $\tau$}

For every finite set $O$ of atomic propositions and every $p \in O$, let
\begin{equation*}
    \ex{p}_O \quad \equiv \quad  p \wedge \bigwedge_{q \in O \smallsetminus \{p\}} \neg q
\end{equation*}


Let $A_i = \{r_i,a_i,b_i,c_i,d_i\}$ for every  $i \in \{0,1,2\}$, and let $A = \bigcup_{i=0}^2 A_i$. Furthermore, for every $i \in \{0,1,2\}$, we use $S(i)$ to denote $i{+}1 \mbox{ mod } 2$.


\begin{eqnarray*}
   \Struct & = & \opg_{=1} \left( \textstyle\bigvee_{p \in A} \ex{p}_{A}\right)\\
       & \wedge &
       \bigwedge_{i=0}^{2} \opg_{=1} \left( 
         r_i \Rightarrow \opf_{=1} (a_i \vee b_i \vee c_i \vee d_i \vee r_{S(i)})
       \right)\\
       & \wedge & 
         \bigwedge_{i=0}^2 \ \bigwedge_{p \in A_i \smallsetminus \{r_i\}} \opg_{=1}\left( p \Rightarrow \opg_{=1} p \right)\\
       & \wedge &
       \bigwedge_{i=0}^2 \opg_{=1} \left( 
            r_i \Rightarrow \opf_{<1} r_{S(i)}\right)
\end{eqnarray*}

\noindent
Observe that $\Struct$ is equivalent to $\opg_{=1} \Struct$, and $\Struct$ implies the formulae
\begin{equation}
   \bigwedge_{i=0}^2 \opg_{=1} \left( r_i \Rightarrow \ex{r_i}_A \opu_{=1} (a_i \vee b_i \vee c_i \vee d_i \vee r_{S(i)})  \right)  
\end{equation}

For every state $t$ such that $t \models r_i$, let $\vec{v}[t] \in [0,1]^2$ be the \emph{characteristic vector of $t$} where
\begin{itemize}
    \item $\vec{v}[t]_1$ is the probability of satisfying 
       $\opg(r_i \vee a_i)$ in $t$;
    \item $\vec{v}[t]_2$ is the probability of satisfying 
       $\opg(r_i \vee b_i)$ in $t$.
\end{itemize}

Let 
\begin{eqnarray}
    \Tau & \equiv & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=\delta}(r_i \vee a_i \vee c_i) )\label{tau-delta1}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=\delta}(r_i \vee S(r_i) \vee c_i) )\label{tau-delta2}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=q}(r_i \vee a_i \vee b_i \vee c_i \vee d_i \vee r_{S(i)} \vee a_{S(i)} )\label{tau-first}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=q}(r_i \vee a_i  \vee c_i \vee d_i \vee r_{S(i)} \vee a_{S(i)} \vee b_{S(i)})\label{tau-second}
\end{eqnarray}

Assume that $t \models r_i \wedge \Struct \wedge \Tau$ and $\vec{v}[t] = \tau^k(\vec{\kappa})$ for some $k \geq 1$. A finite path $t_0,\ldots,t_m$ is \emph{relevant} if $t_0 = t$, $t_j \models r_i$ for all $j<m$, and $t_m \models r_{S(i)}$. We claim that the characteristic vector of the last state $t_m$ of every relevant path satisfies 
$\vec{v}[t_m] = \tau^{k-1}(\vec{\kappa})$. 

The subformulae~\eqref{tau-delta1} and~\eqref{tau-delta2} ensure that the total probability of all relevant finite paths is equal to $\vec{v}[t]_1$. The subformula~\eqref{tau-first} ensures $\vec{v}[t_m]_1 = (q-1+\vec{v}[t]_1)/\vec{v}[t]_1$. The subformulae~\eqref{tau-first} and~\eqref{tau-second}  ensure $\vec{v}[t_m]_2 = \vec{v}[t]_2/\vec{v}[t]_1$.

\subsection{Implementing $\tau$ and $\sigma$}

For every finite set $O$ of atomic propositions and every $p \in O$, let
\begin{equation*}
    \ex{p}_O \quad \equiv \quad  p \wedge \bigwedge_{q \in O \smallsetminus \{p\}} \neg q
\end{equation*}

For every $i \in \{0,1,2\}$, let $\A_i = \{r_i,a_i,b_i,c_i,d_i\}$ and $\B_i = \{R_i,A_i,B_i,C_i,D_i\}$. Furthermore, let $\A = \bigcup_{i=0}^2 \A_i$ and $\B = \bigcup_{i=0}^2 \B_i$. For every $i \in \{0,1,2\}$, we use $S(i)$ to denote $i{+}1 \mbox{ mod } 2$.

Let 
\begin{equation}
\Struct ~~\equiv~~ \opg_{=1} \Psi
\end{equation}
where 

\begin{eqnarray} 
   \Psi & ~~~~\equiv~~~~ & 
       \bigvee_{p \in \A} \ex{p}_{\A} ~~~~\wedge~~~~  \bigwedge_{p \in \A \smallsetminus \{r_0,r_1,r_2\}} p \Rightarrow \opg_{=1} p \\
       & \wedge & 
        \bigvee_{p \in \B} p ~~~~\Rightarrow~~~~ \opg_{=1} \bigvee_{p \in \B} \ex{p}_{\B}
       \\
       & \wedge & 
         \bigwedge_{p \in \B \smallsetminus \{R_0,R_1,R_2\}}  p \Rightarrow \opg_{=1} p\\
       & \wedge & 
         \bigwedge_{i=0}^2 \ \bigwedge_{p \in \A_i \smallsetminus \{a_i,r_i\}} \left( p \Rightarrow \textstyle\bigvee_{q \in \B} q \right)\\
       & \wedge & \bigwedge_{i=0}^2 \ \bigwedge_{p \in \{a_i,r_i\}} \left(p \Rightarrow \ex{p}_{\A \cup\B}\right)\\
       & \wedge &
         \bigwedge_{i=0}^{2} 
           \left(r_i \Rightarrow \opf_{=1} \ASuc_i \right)
         ~~~~\wedge~~~~
         \bigwedge_{i=0}^{2} \left( 
           R_i \Rightarrow \opf_{=1} \BSuc_i
         \right)\\  
       & \wedge &
       \bigwedge_{i=0}^2 \left( 
            r_i \Rightarrow \opf_{<1} r_{S(i)}\right)
        ~~~~\wedge~~~~ 
            \bigwedge_{i=0}^2 \left( 
                 R_i \Rightarrow \opf_{<1} R_{S(i)}\right)
\end{eqnarray}
where
\begin{eqnarray*}
\ASuc_i & \equiv & a_i \vee r_{S(i)} \vee (b_i {\wedge} R_{S(i)}) \vee (c_i {\wedge} R_{S(i)}) \vee (d_i {\wedge} R_{S(i)})\\
\BSuc_i & \equiv & A_i \vee B_i \vee C_i \vee D_i \vee R_{S(i)}
\end{eqnarray*} 

\noindent
Observe that $\Struct$ implies the formulae
\begin{eqnarray}
   && \bigwedge_{i=0}^2 \opg_{=1} \big( r_i ~~\Rightarrow~~ \ex{r_i}_{\A\cup\B} \opu_{=1} \ASuc_i \big)\\
   && \bigwedge_{i=0}^2 \opg_{=1} \big( R_i ~~\Rightarrow~~ \ex{R_i}_{\B} \opu_{=1} \BSuc_i \big)
\end{eqnarray}

For every state $t$ such that $t \models r_i$ or $t \models R_i$, let $\vec{v}[t] \in [0,1]^2$ be the \emph{characteristic vector of $t$} such that
\begin{itemize}
\item If $t \models r_i$, then 
\begin{itemize}
    \item $\vec{v}[t]_1$ is the probability of satisfying 
       $\opg(r_i \vee a_i)$ in $t$;
    \item $\vec{v}[t]_2$ is the probability of satisfying 
       $\opg(r_i \vee b_i)$ in $t$.
\end{itemize}
\item If $t \models R_i$, then 
\begin{itemize}
    \item $\vec{v}[t]_1$ is the probability of satisfying 
       $\opg(R_i \vee A_i)$ in $t$;
    \item $\vec{v}[t]_2$ is the probability of satisfying 
       $\opg(R_i \vee B_i)$ in $t$.
\end{itemize}
\end{itemize}

***************************

Let 
\begin{eqnarray}
    \Tau & \equiv & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=\delta}(r_i \vee a_i \vee c_i) )\label{tau-delta1}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=\delta}(r_i \vee S(r_i) \vee c_i) )\label{tau-delta2}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=q}(r_i \vee a_i \vee b_i \vee c_i \vee d_i \vee r_{S(i)} \vee a_{S(i)} )\label{tau-first}\\
    & \wedge & \bigwedge_{i=0}^2 (r_i \Rightarrow \opg_{=q}(r_i \vee a_i  \vee c_i \vee d_i \vee r_{S(i)} \vee a_{S(i)} \vee b_{S(i)})\label{tau-second}
\end{eqnarray}

Assume that $t \models r_i \wedge \Struct \wedge \Tau$ and $\vec{v}[t] = \tau^k(\vec{\kappa})$ for some $k \geq 1$. A finite path $t_0,\ldots,t_m$ is \emph{relevant} if $t_0 = t$, $t_j \models r_i$ for all $j<m$, and $t_m \models r_{S(i)}$. We claim that the characteristic vector of the last state $t_m$ of every relevant path satisfies 
$\vec{v}[t_m] = \tau^{k-1}(\vec{\kappa})$. 

The subformulae~\eqref{tau-delta1} and~\eqref{tau-delta2} ensure that the total probability of all relevant finite paths is equal to $\vec{v}[t]_1$. The subformula~\eqref{tau-first} ensures $\vec{v}[t_m]_1 = (q-1+\vec{v}[t]_1)/\vec{v}[t]_1$. The subformulae~\eqref{tau-first} and~\eqref{tau-second}  ensure $\vec{v}[t_m]_2 = \vec{v}[t]_2/\vec{v}[t]_1$.


\subsection{An $\opf,\opg$ version of $\Struct$}

We want to define a PCTL state formula $\overline{\Struct}$
in the $\opf,\opg$ fragment of PCTL such that
$\overline{\Struct}$ implies $\Struct$.
%
First, define $\mathcal{C} = \{a_{i,\ell},\bar{a}_{i,\ell},b_{i,\ell},c_{i,\ell},d_{i,\ell} \mid 0\leq i \leq 2, 1\leq \ell \leq m\}$.
%
Now, define $\overline{\Struct}$ as follows:
\[ \overline{\Struct} \equiv \overline{\Succ} \wedge Mark \wedge Lambda, \]
where $Mark$ and $Lambda$ remain as they were in the original $\Struct$
and $\overline{\Succ}$ is defined as follows:
\begin{align*}
  \overline{\Succ} \equiv &
  \bigwedge_{i=0}^{2} \bigwedge_{\ell=1}^{m} \opg_{=1}
  \left(
  \langle r_{i,\ell} \rangle_{\A}
  \implies
  \biggl[ \bigvee_{\ell'=1}^{m} \opf_{=1} rsuc_{i,\ell,\ell'} \biggr]
  \wedge
  \biggl[
    \opf_{<1}
    \bigvee_{\substack{
               0 \leq z \leq 2 \\
               1 \leq z' \leq m \\
               z \neq i \text{ or } z' \neq \ell}
              }
    \ex{r_{z,z'}}_{\A} 
  \biggr]
  %\biggl[ \opf_{<1}
  %  \bigvee_{\substack{0 \leq j \leq 2 \\ j \neq i}}
  %  \bigvee_{\substack{1 \leq k \leq m \\ k \neq \ell}}
  %  r_{j,k}
  %\biggr]
  %\biggl[
  %  \bigwedge_{\substack{0 \leq j \leq 2 \\
  %             1 \leq k \leq m \\
  %             k \neq \ell \text{ or } j \neq i}
  %            }
  %  \bigwedge_{\substack{1 \leq u \leq m}}
  %  \opf_{<1} rsuc_{j,k,u}
  %\biggr]
  \right) \\
  & \wedge \\
  & \opg_{=1} \bigvee_{x \in \A \setminus \B} \ex{x}_{\A \setminus \B} \\
  & \wedge \\
  & \opg_{=1} \bigwedge_{x \in \mathcal{C}} \left( x \implies \bigvee_{0 \leq j \leq 2} \ex{x,R_j}_{\A} \right) \\
  & \wedge \\
  & \opg_{=1} \bigwedge_{x \in \A \setminus (\B \cup \mathcal{C})} \left( x \implies \ex{x}_{\A} \right) \\
  %& \wedge \\
  %& \opg_{=1} \left( \bigvee_{x \in \B} x \implies \opg_{=1} \bigvee_{x \in \B} x \right) \\
  % FIXME stuff for the second conjunct.
\end{align*}

It is easy to see that $\overline{\Struct}$ is a PCTL state formula 
in the $\opf,\opg$ fragment of PCTL. It remains to show
$\overline{\Struct}$ implies $\Struct$.

Suppose that $\overline{\Struct}$ holds in some state $o$.
We want to show that $\Struct$ also holds in $o$.
Clearly $Mark$ and $Lambda$ are satisfied,
so it remains to show that $\Succ$ is satisfied.
Recall the definition of $\Succ$:
\begin{eqnarray*}\\[-2em]
    \Succ & \equiv & \bigwedge_{\ell=1}^m \bigwedge_{i=0}^2 \opg_{=1} \bigg(  \ex{r_{i,\ell}}_{\A} \ \Rightarrow \ \bigvee_{\ell'=1}^m \ex{r_{i,\ell}}_{\A} \opu_{=1} \rSuc_{i,\ell,\ell'} \bigg)\\ 
       & \wedge & \bigwedge_{i=0}^2 \opg_{=1} \bigg(
       \big( \ex{R_i}_{\B} \ \Rightarrow \ \ex{R_i}_{\B} \opu_{=1} \RSuc_i \big) 
       \wedge
       \big( \ex{R_i,K}_{\B} \ \Rightarrow \ \ex{R_i,K}_{\B} \opu_{=1} \RKSuc_i \big) 
       \bigg)
\end{eqnarray*}
where\\[-2.5em]
\begin{eqnarray*}
    \rSuc_{i,\ell,\ell'} & \equiv & \ex{r_{S(i),\ell'}}_{\A} \vee \bigvee_{j=0}^2 \left(\ex{a_{i,\ell},R_j}_{\A} \ \vee \ex{\bar{a}_{i,\ell},R_j}_{\A}\ \vee \ \ex{b_{i,\ell}, R_j}_{\A} \ \vee \ \ex{c_{i,\ell},R_j}_{\A} \ \vee \ \ex{d_{i,\ell},R_j}_{\A}\right)  \\
    \RSuc_i & \equiv & \ex{A_i}_{\B} \ \vee \ \ex{B_i}_{\B} \ \vee \ \ex{C_i}_{\B} \ \vee \ \ex{D_i}_{\B} \ \vee \ \ex{E_i}_{\B} \ \vee \ \ex{R_{S(i)},K}_{\B}\\
    \RKSuc_i & \equiv & \ex{A_i,K}_{\B} \ \vee \ \ex{B_i,K}_{\B} \ \vee \ \ex{C_i,K}_{\B} \ \vee \ \ex{D_i,K}_{\B}  \ \vee \ \ex{R_{S(i)},K}_{\B}.
\end{eqnarray*} 

We will first show that its first conjunct,
\[
\bigwedge_{\ell=1}^m \bigwedge_{i=0}^2 \opg_{=1} \bigg(  \ex{r_{i,\ell}}_{\A} \ \Rightarrow \ \bigvee_{\ell'=1}^m \ex{r_{i,\ell}}_{\A} \opu_{=1} \rSuc_{i,\ell,\ell'} \bigg),
\]
is satisfied in $o$.

Let $\ell \in \{1, \ldots, m\}$ and $i \in \{ 0, \ldots, 2 \}$.
Suppose $\ex{r_{i,\ell}}_{\A}$ is satisfied in some state $s$ that
is reachable from $o$.
We want to show that $s$ satisfies
\[
\bigvee_{\ell'=1}^m \ex{r_{i,\ell}}_{\A} \opu_{=1} \rSuc_{i,\ell,\ell'}.
\]
We know that $o$ satisfies $\overline{\Succ}$, and since $s$ is a state
reachable from $o$ that satisfies $\ex{r_{i,\ell}}_{\A}$,
it is easy to see that $s$ must satisfy
\[
\bigvee_{\ell'=1}^{m} \opf_{=1} rsuc_{i,\ell,\ell'}.
\]
Then $s$ satisfies $\opf_{=1} rsuc_{i,\ell,\ell'}$ for some
$\ell' \in \{ 1, \ldots, m \}$. Fix such $\ell'$.
We will show that $s$ satisfies
\[
\ex{r_{i,\ell}}_{\A} \opu_{=1} \rSuc_{i,\ell,\ell'}.
\]
We will do so by showing that every path $\pi$ starting in $s$
that satisfies $\opf rsuc_{i,\ell,\ell'}$ also satisfies
$\ex{r_{i,\ell}}_{\A} \opu \rSuc_{i,\ell,\ell'}$.


Let $\pi$ be a path that starts in $s$ and satisfies
$\opf rsuc_{i,\ell,\ell'}$.
%
Then there exists $\alpha \in \nat$ such that $\pi(\alpha)$ satisfies
$rsuc_{i,\ell,\ell'}$.
%
Let $\alpha$ be the least such $\alpha$.
%
It is now sufficient to show that $\pi(\beta)$ satisfies $\ex{r_{i,\ell}}_{\A}$ for every $\beta \in \nat$ such that $\beta < \alpha$.


Suppose it does not.
%
Then there exists $\beta \in \nat$ such that $\beta < \alpha$ and $\pi(\beta)$ does not satisfy $\ex{r_{i,\ell}}_{\A}$.
%
Let $\beta$ be such $\beta$.
%
Since $o$ satisfies \( \overline{\Succ} \),
we know that $\pi(\beta)$ satisfies \(\ex{x}_{\A \setminus \B}\) for some \(x \in \A \setminus \B\).
%
Let $x$ be such $x$.


We will now show that $x \not \in \mathcal{C}$, by contradiction.
%
Suppose that $x \in \mathcal{C}$.
%
Since $o$ satisfies \( \overline{\Succ} \),
it follows that $\pi(\beta)$ satisfies $\ex{x,R_j}_{\A}$ for some $0 \leq j \leq 2$.
%
Recall that $x \in \mathcal{C}$ and 
$\mathcal{C} = \{a_{i,\ell},\bar{a}_{i,\ell},b_{i,\ell},c_{i,\ell},d_{i,\ell} \mid 0\leq i \leq 2, 1\leq \ell \leq m\}$.
%
Then there exist $j,k \in \nat$ such that
$0 \leq j \leq 2$ and $1 \leq k \leq m$ and
$x$ is one of $a_{j,k}$, $\bar{a}_{j,k}$,
$b_{j,k}$, $c_{j,k}$, $d_{j,k}$.
%
Fix such $j$ and $k$.
%
It is easy to see that $j \neq i$ or $k \neq \ell$,
otherwise $\pi(\beta)$ would satisfy $rsucc_{i,l,\ell}$, a contradiction.
%
Recall that $\pi(\beta)$ satisfies \( \ex{x}_{\A \setminus \B} \)
and $x \in \mathcal{C}$.
%
Observe that $\{x\}$ is a $\A \setminus \B$ marker for every $x \in \mathcal{C}$.
%
Given that $\pi(\alpha)$ is obviously reachable from $\pi(\beta)$,
it follows that $\pi(\alpha)$ satisfies \( \ex{x}_{\A \setminus \B} \).
%
We already know that $x$ is one of $a_{j,k}$, $\bar{a}_{j,k}$,
$b_{j,k}$, $c_{j,k}$, $d_{j,k}$ and that $j \neq i$ or $k \neq \ell$.
%
It follows that $\pi(\alpha)$ does not satisfy $rsucc_{i,\ell,\ell'}$,
a contradiction.
%
In conclusion, $x \not \in \mathcal{C}$.


We have now established that $x \not \in \mathcal{C}$.
%
By its definition, $x \in \A \setminus \B$.
%
Therefore, $x \in \A \setminus (\B \cup \mathcal{C})$.
%
Since $o$ satisfies $\opg_{=1} \bigwedge_{x \in \A \setminus (\B \cup \mathcal{C})} \left( x \implies \ex{x}_{\A} \right)$ and $\pi(\beta)$ satisfies $x$,
it follows that $\pi(\beta)$ satisfies $\ex{x}_{\A}$.
%
Since $x \in \A \setminus \B$ and $x \not \in \mathcal{C}$,
$x$ must be $r_{j,k}$ for some $j,k \in \nat$ such that
$0 \leq j \leq 2$ and $1 \leq k \leq m$.
%
Fix such $j,k$.
%
We now know that $\pi(\beta)$ satisfies $\ex{r_{j,k}}_{\A}$.
%
Observe that $j \neq i$ or $k \neq \ell$,
otherwise $\pi(\beta)$ would satisfy $\ex{r_{i,\ell}}_{\A}$,
contradicting the definition of $\beta$.
%
Observe that $o$ satisfies $\overline{\Succ}$ and $\pi(\beta)$
is reachable from $o$ and $\pi(\beta)$ satisfies $\ex{r_{j,k}}_{\A}$.
%
It follows that $\pi(\beta)$ satisfies $\opf_{=1} rsuc_{j,k,k'}$ for some $1 \leq k' \leq m$.
%
Fix such $k'$.



We will now show that $\pi(\beta)$ satisfies
$\opf_{=1} rsuc_{i,\ell,\ell'}$.
%
Recall that $s$ satisfies $\opf_{=1} rsuc_{i,\ell,\ell'}$.
%
Also recall that $\pi$ is a path starting in $s$, so $\pi(0) = s$.
%
From the definition of $\alpha$, we know that $\pi(\gamma)$ does not
satisfy $rsuc_{i,\ell,\ell'}$ for every $\gamma \in \nat$ such
that $\gamma \leq \beta$.
%
Now it is easy to see that if $\pi(\beta)$ did not satisfy
$\opf_{=1} rsuc_{i,\ell,\ell'}$, neither would $s$, a contradiction.
%
In conclusion, $\pi(\beta)$ satisfies $\opf_{=1} rsuc_{i,\ell,\ell'}$.



We have now established that $\pi(\beta)$ satisfies
$\opf_{=1} rsuc_{i,\ell,\ell'}$ and
$\opf_{=1} rsuc_{j,k,k'}$.
%
We also have already established that $j \neq i$ or $\ell \neq k$.
%
Recall that $\pi(\beta)$ satisfies $\ex{r_{j,k}}_{\A}$.
%
Recall that $o$ satisfies $\overline{\Succ}$,
and so it follows that $\pi(\beta)$ must also satisfy
\[
    \opf_{<1}
    \bigvee_{\substack{
               0 \leq z \leq 2 \\
               1 \leq z' \leq m \\
               z \neq j \text{ or } z' \neq k}
              }
    \ex{r_{z,z'}}_{\A}.
\]
%
Let $\pi'$ be a path starting in $\pi(\beta)$ that
satisfies $\opf rsuc_{j,k,k'}$.
%
Let $\gamma \in \nat$ be the least natural number such that $\pi'$
satisfies $rsuc_{j,k,k'} \vee rsuc_{i,\ell,\ell'}$ (it is easy
to see that such $\gamma$ exists).
%
It is easy to see that if $\pi'(\gamma)$ satisfied one of
$a_{i,\ell}$, $\bar{a}_{i,\ell}$, $b_{i,\ell}$, $c_{i,\ell}$, $d_{i,\ell}$,
then $\pi'$ could not satisfy $\opf rsuc_{j,k,k'}$, a contradiction.
%
It is not hard to see that if $\pi'(\gamma)$ satisfied one of
$a_{j,k}$, $\bar{a}_{j,k}$, $b_{j,k}$, $c_{j,k}$, $d_{j,k}$,
then $\pi(\beta)$ could not satisfy $\opf_{=1} rsuc_{i,\ell,\ell'}$,
a contradiction.
%
Therefore, $\pi'(\gamma)$ satisfies $\ex{r_{S(i),\ell'}}_{\A}
\vee \ex{r_{S(j),k'}}_{\A}$.
%
%Note that if $S(i)=j$ and $\ell'=k$, then $\pi(\beta)$ satisfies
%$\ex{r_{S(i),\ell'}}_{\A}$, which means $\pi(\beta)$ satisfies
%$rsuc_{i,\ell,\ell'}$, a contradiction.
%
It follows that $\pi'(\gamma)$ satisfies 
\[
    \bigvee_{\substack{
               0 \leq z \leq 2 \\
               1 \leq z' \leq m \\
               z \neq j \text{ or } z' \neq k}
              }
    \ex{r_{z,z'}}_{\A}.
\]
%
Therefore, every path starting in $\pi(\beta)$ that
satisfies $\opf rsuc_{j,k,k'}$ also satisfies
\[
    \opf
    \bigvee_{\substack{
               0 \leq z \leq 2 \\
               1 \leq z' \leq m \\
               z \neq j \text{ or } z' \neq k}
              }
    \ex{r_{z,z'}}_{\A}.
\]
%
We already know that $\pi(\beta)$ satisfies
$\opf_{=1} rsuc_{j,k,k'}$, and so it follows that
$\pi(\beta)$ also satisfies 
\[
  \opf_{=1}
    \bigvee_{\substack{
               0 \leq z \leq 2 \\
               1 \leq z' \leq m \\
               z \neq j \text{ or } z' \neq k}
              }
    \ex{r_{z,z'}}_{\A},
\]
which is a contradiction.


==> minsky.tex <==
\section{Simulating Minsky Machines with Two Counters}
\label{sec-Minsky-simulation}

In this section, we show how to simulate non-deterministic two-counter Minsky machines by  PCTL formulae. Technically, we construct a PCTL formula simulating a synchronized products of two non-deterministic one-counter Minsky machines defined in the next paragraph.

Let 
\begin{eqnarray*}
   \M_1 & \equiv & 1:\Ins_1^1;\cdots m: \Ins_m^1;\\ 
   \M_2 & \equiv & 1:\Ins_1^2;\cdots m: \Ins_m^2;
\end{eqnarray*}
be nondetermnistic one-counter Minsky machines with $m$ instructions and $I = (I_1,I_2)$ a partition of $\{1,\ldots,m\}$, i.e., $I_1 \cup I_2 = \{1,\ldots,m\}$ and $I_1 \cap I_2 = \emptyset$. An \emph{$I$-synchronized product} of $\M_1,\M_2$, denoted by $\M_1 \times_I \M_2$, is an automaton\footnote{$\M_1 \times_I \M_2$ is a non-standard computational model introduced specifically for purposes of this paper. Encoding the computation of $\M_1 \times_I \M_2$ by a PCTL formula is substantially easier than encoding the computation of a two-counter Minsky machine.} operating over two counters in the following way.

A \emph{configuration} of $\M_1 \times_I \M_2$ is a triple $(j,n_1,n_2)$ where $j \in \{1,\ldots,m\}$ and $n_1,n_2 \in \N$ are counter values. For every configuration $(j,n_1,n_2)$ of $\M_1 \times_I \M_2$, the \emph{successor} configurations $(j',n_1',n_2')$ are determined as follows (recall that $\mapsto$ denotes the ``standard'' computational step of a Minsky machine, see Section~\ref{sec-Minsky}):

\begin{itemize}
    \item If $j \in I_1$, then $j',n_1',n_2'$ are integers satisfying $(j,n_1) \mapsto (j',n_1')$ in $\M_1$ and $(j,n_2) \mapsto (j'',n_2')$ in $\M_2$ (for some $j'' \in \{1,\ldots,m\}$).
    \item If $j \in I_2$, then $j',n_1',n_2'$ are integers satisfying $(j,n_1) \mapsto (j'',n_1')$ in $\M_1$ and $(j,n_2) \mapsto (j',n_2')$ in $\M_2$ (for some $j'' \in \{1,\ldots,m\}$).
\end{itemize}

In other words, $\M_1 \times_I \M_2$ simultaneously executes the instructions $\Ins^1_j$ and $\Ins^2_j$ operating on the first and the second counter, and the next $j'$ is determined by either $\Ins^1_j$ or $\Ins^2_j$, depending on whether $j \in I_1$ or $j \in I_2$, respectively.
Note that the counter values $n_1'$ and $n_2'$ are the \emph{same} in every successor configuration of $(j,n_1,n_2)$.

We write $(j,n_1,n_2) \leadsto (j',n_1',n_2')$ when $(j',n_1',n_2')$ is a successor of $(j,n_1,n_2)$. A \emph{computation} of $\M_1 \times_I \M_2$ is an infinite sequence of configurations $\omega \equiv D_0,D_1,\ldots$ such that $D_i \leadsto D_{i+1}$ for all $i \in \N$. The boundedness and the recurrent reachability problems for \mbox{$\M_1 \times_I \M_2$} are defined in the same way as for non-deterministic Minsky machines (see Section~\ref{sec-Minsky}). 

A synchronized product of two one-counter Minsky machines can faithfully simulate a two-counter Minsky machine. Thus, we obtain the following:

\begin{restatable}{proposition}{Minskyproduct}
\label{prop-product}
    The boundedness problem for a synchronized product of two deterministic one-counter Misky machines is $\Sigma_1^0$-hard. The recurrent reachability problem for a synchronized product of two non-deterministic one-counter Misky machines is $\Sigma_1^1$-hard.
\end{restatable}
 
%also reveals that we can safely assume that both counters are zero when $\M_1 \times_I \M_2$ reaches a halting configuration $(m{+}1,n_1,n_2)$.

Let $\M_1 \times_I \M_2$ be a synchronized product of two non-deterministic one-counter Misky machines with~$m$ instructions. Recall the set $\A$ defined in Section~\ref{sec-one-counter-psi}. For $k \in \{1,2\}$, let $\A^k = \{p^k \mid p \in \A\}$ be a set of atomic propositions such that $\A^1 \cap \A^2 = \emptyset$.



Let $M = (S,P,v)$ be a Markov chain. For all $t \in S$ and $k \in \{1,2\}$, we use $\vec{v}^k[t] \in [0,1]^2$ to denote the $k$-th characteristic vector of $t$ where
\begin{itemize}
    \item $\vec{v}^k[t]_1$ is the probability of satisfying the path formula $\opx a^k$ in the state~$t$;
    \item $\vec{v}^k[t]_2$ is the probability of satisfying the path formula $\opx b^k$ in the state~$t$.
\end{itemize}
A state $t \in S$ \emph{represents a configuration $(i,n_1,n_2)$} of $\M_1 \times_I \M_2$ iff $t \models \ell^1_i \wedge \ell^2_i$, $t \not\models \ell_j^1 \wedge \ell_j^2$ for all $j \neq i$, $\vec{v}^1[t] = \sigma^{n_1}(\vec{\kappa})$, and $\vec{v}^2[t] = \sigma^{n_2}(\vec{\kappa})$. Furthermore, we say that a state $s \in S$ \emph{simulates $\M_1 \times_I \M_2$} if $s$ represents $(1,0,0)$ and every state $t$ reachable from~$s$ satisfies the following condition: If $t$ represents a configuration $D$ of $\M_1 \times_I \M_2$, then at least one immediate successor of $t$ represents a successor configuration of~$D$. Furthermore, for every immediate successor $t'$ of $t$ that does \emph{not} represent a successor of $D$ we have that $t' \models \opg_{=1} \bigwedge_{i=1}^m \neg(\ell_i^1 \wedge \ell_i^2)$. 

Let $s \in S$ be a state simulating $\M_1 \times_I \M_2$, and let $s_0,s_1,\ldots$ be a run of $M$ such that $s_0 = s$ and every $s_i$ represents a configuration $D_i$ of $\M_1 \times_I \M_2$. Then $D_0,D_1,\ldots$ is a computation of $\M_1 \times_I \M_2$ \emph{covered by $s$}. 

Now, we formulate the main technical result of this paper. 

\begin{theorem}
\label{thm-two-counter}
Let $\M_1 \times_I \M_2$ be a synchronized product of two non-deterministic one-counter Minsky machines. Then there is an effectively constructible PCTL formula $\Psi$ satisfying the following conditions:
\begin{itemize}
    \item[(A)] For every Markov chain $M$ and every state $s$ of $M$, we have that if $s \models \Psi$, then $s$ simulates $\M_1 \times_I \M_2$.
    \item[(B)] For every computation $\omega$ of $\M_1 \times_I \M_2$, there exists a Markov chain $M$ and a state $s$ of $M$ such that $s \models \Psi$ and $s$ covers $\omega$. 
    Furthermore, if $\omega$ is periodic, then $M$ has finitely many states.
\end{itemize}
\end{theorem}

Observe the following:
\begin{itemize}
    \item Let $\M_1 \times_I \M_2$ be a synchronized product of two \emph{deterministic} one-counter Minsky machines. Then, $\M_1 \times_I \M_2$ is bounded iff the only computation $\omega$ of $\M_1 \times_I \M_2$ is periodic. By Theorem~\ref{thm-two-counter}, we obtain that $\M_1 \times_I \M_2$ is bounded iff $\Psi$ is finite-satisfiable.
    \item Let $\M_1 \times_I \M_2$ be a synchronized product of two \emph{non-deterministic} one-counter Minsky machines. Then \mbox{$\M_1 \times_I \M_2$} has a recurrent computation iff the formula 
    \begin{equation*}
        \Psi \ \wedge \ \opg_{=1} \left( (\ell_1^1 \wedge \ell_1^2) \Rightarrow \opf_{>0} (\ell_1^1 \wedge \ell_1^2)\right)
    \end{equation*}
    is (generally) satisfiable.
\end{itemize} 

Thus, we obtain the following corollary to Theorem~\ref{thm-two-counter}:

\begin{corollary}
    The finite satisfiability problem for PCTL is \mbox{$\Sigma_1^0$-hard}, and the general satisfiability problem pro PCTL is \mbox{$\Sigma_1^1$-hard}.
\end{corollary}

\subsection{Constructing $\Psi$}
\label{sec-two-counters-formula}

For the rest of this section, we fix the following non-deterministic one-counter Minsky machines:
\begin{eqnarray*}
    \M_1 & \equiv & 1:\Ins_1^1;\cdots m: \Ins_m^1;\\ 
    \M_2 & \equiv & 1:\Ins_1^2;\cdots m: \Ins_m^2;
 \end{eqnarray*}
Furthermore, we fix a partition $I = (I_1,I_2)$ of $\{1,\ldots,m\}$. 

Roughly speaking, the formula $\Psi$ is obtained by ``merging'' the formulae $\psi_1$ and $\psi_2$ of Section~\ref{sec-counter} constructed for $\M_1$ and $\M_2$ using the disjoint sets of atomic propositions $\A^1$ and $\A^2$. The main modification is in the subformulae $\LTrans$ of $\psi_1$ and $\psi_2$, where we need to adjust the way of selecting the propositions of $\Labels$ passed to the successors so that the operational semantics of $\M_1 \times_I \M_2$ is reflected properly. When constructing $\psi_1$ and $\psi_2$, we assume the constants $q$, $\vec{\kappa}$, and $\gamma$ satisfying the same constraints as in Section~\ref{sec-counter} (these constants are used in both $\psi_1$ and $\psi_2$).

The set of atomic propositions used in $\Psi$ is $\A^1 \cup \A^2$. For every formula $\textit{Form}$ constructed in Section~\ref{sec-counter} and $k \in \{1,2\}$, we use $\textit{\textbf{Form}}^k$ to denote the formula obtained from $\textit{Form}$ by replacing all propositions of $\A$ with $\A^k$. For example, $t \models \pmb{\Ex{a,r_i}}^1$ if $t$ satisfies both $a^1$ and $r_i^1$, and no other proposition of $\A^1$. The formula does not say anything about 
the validity of the propositions of $\A^2$ in~$t$.

When we need to define new formulae over $\A^1$ and $\A^2$ with the same structure up to the upper indexes of atomic propositions, we write a definition of $\textit{Form}^k$ parameterized by the~$k$. For example, by stipulating $\textit{Form}^k \equiv h^k \vee \pmb{\Ex{a,r_i}}^k$, we simultaneously define $\textit{Form}^1 \equiv h^1 \vee \pmb{\Ex{a,r_i}}^1$ and $\textit{Form}^2 \equiv h^2 \vee \pmb{\Ex{a,r_i}}^2$.
Furthermore, for $k \in \{1,2\}$, the other element of $\{1,2\}$ is denoted by $k'$, i.e., $\{k,k'\} = \{1,2\}$. 

We put
\[
     \Psi \ \equiv \ \bInit^1 \wedge \bInit^2 \wedge \opg_{=1} (\Invariant \wedge \LPass)   
\]
where
\begin{eqnarray*}
   \LPass & \equiv & \ \left(\bigvee_{j=1}^m (\ell^1_j \wedge \ell^2_j)\right) \ \Rightarrow \ \opx_{>0}\left( \bigvee_{j=1}^{m} (\ell^1_j \wedge \ell^2_j)\right)\\[1ex]
%    \Disjoint & \equiv & \left( \bigwedge_{j=1}^{m+1} (\neg \ell_j^1 \vee \neg \ell_j^2)\right)
%    \Rightarrow \left( \bigwedge_{a \in \A^1} \neg p \ \vee\ \bigwedge_{a \in \A^2} \neg p \right)
    \Invariant  & \equiv & (\bFin^1 \vee \Transient^1 \vee \bFree^1)\\
    & \wedge & (\bFin^2 \vee \Transient^2 \vee \bFree^2)
\end{eqnarray*}
Intuitively, if $t \models \ell_j^1 \wedge \ell_j^2$, then the instructions $\Ins_j^1$ 
and $\Ins_j^2$ are ``simulated in parallel'' in $t$. The formula $\LPass$ enforces 
the existence of at least one immediate successor $t'$ of $t$ where the successor instructions  $\Ins_{j'}^1$ and $\Ins_{j'}^2$ are again simulated jointly. 
%The formula $\Disjoint$ says that all other states satisfy only the propositions of $\A^1$ or only the propositions of $\A^2$.
%Note that if $s \models \Psi$, then $s \models \ell_1^1 \wedge \ell_1^2$. 
For all $k \in \{1,2\}$, we put
\begin{eqnarray*}
    \Transient^k &  \equiv & \bTrans^k \vee \bCTrans^k \vee \LTrans^k
\end{eqnarray*}
where
\begin{eqnarray*}
    \LTrans^k &  \equiv & \bigg(\bigvee_{j=1}^m (\ell_j^k \wedge  \ell_j^{k'}) \bigg) \Rightarrow \Simulate^k\\
    & \wedge & \bigg(\bigvee_{j=1}^m (\ell_j^k  \wedge   \neg \ell_j^{k'}) \bigg) \Rightarrow \Abandon^k
\end{eqnarray*}

As we shall see, for every state $t$ reachable from a state satisfying $\Psi$ we have that $t \models \ell_j^k$ for at most one $\ell_j \in \Labels$. Intuitively, the formula $\LTrans^k$ says that when $t \models \ell_j^k \wedge \ell_j^{k'}$, we continue with simulating the instruction $\Ins_j^k$. If $t$ satisfies a proposition $\ell_j^k \in \Labels^k$ but not the matching proposition $\ell_j^{k'} \in \Labels^{k'}$, we ``abandon'' the simulation. In the latter case, the immediate successors of $t$ must still have an appropriate structure so that no formula is ``spoilt'' in the immediate predecessor of~$t$. This is enforced by the formula $\Abandon^k$. More precisely, we put
\begin{eqnarray*}
\Abandon^k & \equiv & (\bZero^k \Rightarrow \OZer^k)
             \wedge  (\neg\bZero^k \Rightarrow \OPos^k)\,.
\end{eqnarray*}
The formulae $\OZer^k$ and $\OPos^k$ are defined as follows:
\begin{eqnarray*}
    \OZer^k & \equiv & \bigvee_{i \in \{0,\ldots,4\}}  ( r_i^k \wedge \OZsuc^k_i)\\  
    \OPos^k & \equiv & 
    \bigvee_{i \in \{0,\ldots,4\}} ( r_i^k \wedge \OPsuc_i^k \wedge \bInterval^k \wedge \bEq_i^k )
\end{eqnarray*}
where
\begin{eqnarray*}  
    \OZsuc^k_i & \equiv & \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k 
            \vee \pmb{\Ex{h,c,S^2(r_i)}}^k\\
    && \hspace*{5ex}  \vee\ \pmb{\Ex{h,c,S^2(r_i),e}}^k\big) \ \wedge \ 
    \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}}^k \\
    \OPsuc^k_i & \equiv & \opx_{=1} \big(\pmb{\Ex{a,S(r_i)}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k 
    \vee \pmb{\Ex{h,c,S^2(r_i)}}^k\\
&& \hspace*{5ex}  \vee\ \pmb{\Ex{h,c,S^2(r_i),e}}^k\big) \ \wedge \ 
\opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}}^k
\end{eqnarray*}

The formulae $\Simulate^k$, where $k \in \{1,2\}$, enforce the simulation of one computational step of $\M_1 \times_I \M_2$.
We put
\begin{eqnarray*}   
    \Simulate^k & \equiv &\bigvee_{i \in \{0,\ldots,4\}} \bigvee_{\ell \in \Labels} \bigvee_{x \in \{a,b\}} 
    \  \left(\pmb{\Ex{x,r_i,\ell}}^k \wedge \NStep^k_{i,\ell}\right)
\end{eqnarray*}
where the formula $\NStep^k_{i,\ell}$ is constructed as follows. Let $\Ins_j^k$ be the instruction associated with $\ell$, i.e., $\ell = \ell_j$. If $j \in I_k$, then
\[
    \NStep^k_{i,\ell} \ \equiv \bStep^k_{i,\ell}    
\]

Now let $j \not\in I_k$. For every $L \subseteq \Labels$ where $L$ has one or two elements, let $\bStep^k_{i,\ell}[L]$ be the formula obtained from $\bStep^k_{i,\ell}$ by substituting every occurrence of every set of target labels with $L^k = \{p^k \mid p \in L\}$. Note that this substitution affects only the ``big disjunction'' in the subformulae $\bZsuc_{i,\ell}^k$, $\bPsuc_{i,\ell}^k$, $\bIZsuc_{i,\ell}^k$, and $\bIPsuc_{i,\ell}^k$. Now, we distinguish two cases (recall that $k' \neq k$ is ``the other index'' of $\{1,2\}$).
\smallskip

(A) $\Ins_j^{k'} \equiv \textit{if } c{=}0 \textit{ then goto } L \textit{ else dec } c; \textit{ goto } L'$. Then,
\begin{eqnarray*}
    \NStep_{i,\ell}^k & \equiv &  \left(\bZero^{k'} \Rightarrow \bStep^k_{i,\ell}[L]\right)
     \wedge \ \left(\neg \bZero^{k'} \Rightarrow \bStep^k_{i,\ell}[L']\right)\\
\end{eqnarray*}

(B) $\Ins_j^{k'} \equiv \textit{inc } c; \textit{ goto } L$. Then,
\begin{eqnarray*}
    \NStep_{i,\ell}^k & \equiv &  \bStep^k_{i,\ell}[L]
\end{eqnarray*}
This completes the construction of $\Psi$.

% \smallskip

% \noindent
% (A)  If $\Ins_j^k \equiv \textit{if } c{=}0 \textit{ then goto } u \textit{ else dec } c; \textit{ goto } u'$, then
% \begin{eqnarray*}
%         \Step_{i,\ell,x}^k & \equiv & \hspace*{2ex} \left(\bZero^k \Rightarrow (\Zsuc_{i,\ell,x}^k \wedge \opx_{=1} (b^k \Rightarrow \bZero^k))\right)\\
%         && \wedge \left( \neg\bZero^k \Rightarrow (\Psuc_{i,\ell,x}^k \wedge \bInterval^k \wedge \bEq_i^k ) \right)
% \end{eqnarray*}
% where the formulae $\Zsuc_{i,\ell,x}^k$ and $\Psuc_{i,\ell,a}^k$ depend on the instruction $\Ins_{j}^{\widehat{k}}$ performed by $\M_{\widehat{k}}$. There are two subcases:

%     (Aa) If $\Ins_j^{\widehat{k}} \equiv \textit{if } c{=}0 \textit{ then goto } w \textit{ else dec } c; \textit{ goto } w'$, then  
%     \begin{eqnarray*}
%         \Zsuc_{i,\ell,a}^k & \equiv & \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_w}} \vee
%                                  \pmb{\Ex{h,c,S^2(r_i)}}^k\big)\\  
%                            & \wedge & \neg  \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_{w'}}} \vee
%                            \pmb{\Ex{h,c,S^2(r_i)}}^k\big)\\                    
%         \Zsuc_{i,\ell,b}^k & \equiv & \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_w}}^k \vee
%                                  \pmb{\Ex{h,c,S^2(r_i)}}^k\\
%         && \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k\big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}^k}\\ 
%                            & \wedge & \neg  \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_{w'}}}^k \vee
%                            \pmb{\Ex{h,c,S^2(r_i)}}^k\\ 
%         && \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k\big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}^k}\\  
%         \Psuc_{i,\ell,a}^k & \equiv & \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k \big)\\
%                       & \wedge & \neg  \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w'}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k \big)\\
%         \Psuc_{i,\ell,b}^k & \equiv & \bZero^{\widehat{k}} \Rightarrow \\    
%         && \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k\\
%         &&  \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k \big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}}^k\\
%                         & \wedge & \neg  \bZero^{\widehat{k}} \Rightarrow \\
%         && \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w'}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k\\
%         &&  \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k \big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}}^k\\
%     \end{eqnarray*}
    
%     (Ab) If $\Ins_j^{\widehat{k}} \equiv \textit{inc } c; \textit{ goto } w$, then
%     \begin{eqnarray*}
%         \Zsuc_{i,\ell,a}^k & \equiv & 
%          \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_w}} \vee
%                                  \pmb{\Ex{h,c,S^2(r_i)}}^k\big)\\             
%         \Zsuc_{i,\ell,b}^k & \equiv & 
%          \opx_{=1} \big(\pmb{\Ex{h,a,S(r_i)}}^k \vee \pmb{\Ex{b,S^2(r_i),\ell_w}}^k \vee
%                                  \pmb{\Ex{h,c,S^2(r_i)}}^k\\
%         && \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k\big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}^k}\\ 
%         \Psuc_{i,\ell,a}^k & \equiv & 
%          \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k \big)\\
%         \Psuc_{i,\ell,b}^k & \equiv & 
%          \opx_{=1} \big(\pmb{\Ex{a,S(r_i),\ell_{w}}}^k \vee \pmb{\Ex{h,b,S^2(r_i)}}^k \vee \pmb{\Ex{h,c,S^2(r_i)}}^k\\
%         &&  \hspace*{5ex} \vee \ \pmb{\Ex{h,c,S^2(r_i),e}}^k \big) \ \wedge \ \opx_{=1{-}q} \pmb{\Ex{h,c,S^2(r_i),e}}^k\\
%     \end{eqnarray*}
    

\subsection{A Proof of Theorem~\ref{thm-two-counter}}

% For every state $t$ of some Markov chain and every $k \in \{1,2\}$, we use $\vec{v}^k[t] \in [0,1]^2$ to denote the $k$-th characteristic vector of $t$ where
% \begin{itemize}
%     \item $\vec{v}^k[t]_1$ is the probability of satisfying the path formula $\opx a^k$ in the state~$t$;
%     \item $\vec{v}^k[t]_2$ is the probability of satisfying the path formula $\opx b^k$ in the state~$t$.
% \end{itemize}


% Theorem~\ref{thm-PCTL-undec} is a consequence of the following propositions. 

% \begin{proposition}
% \label{prop-Minsky-unbounded}
% Let $M =(S,P,v)$ be a finite-state model of~$\Psi$. Then for every reachable configuration $(j,n_1,n_2)$ of $\M_1 \times_I \M_2$, there is $t \in S$ such that $t \models \ell^1_j \wedge \ell_j^2$, $\vec{v}^1[t] = \sigma^{n_1}(\vec{\kappa})$, and $\vec{v}^2[t] = \sigma^{n_2}(\vec{\kappa})$.
% \end{proposition}

% \begin{proposition}
% \label{prop-Minsky-bounded}   
% If $\M_1 \times_I \M_2$ is bounded, then $\Psi$ has a finite-state model.
% \end{proposition}

Theorem~\ref{thm-two-counter} is proven by reusing the arguments used in the proof of Theorem~\ref{thm-one-counter}  with some modifications and extensions. Let 
$\M_1 \times_I \M_2$ be a synchronized product of two non-deterministic one-counter Minsky machines with $m$~instructions, and let $\Psi$ be the formula constructed for $\M_1 \times_I \M_2$ in Section~\ref{sec-two-counters-formula}. The two claims of Theorem~\ref{thm-two-counter} are proven separately in the following subsections.

\subsubsection{A Proof of Theorem~\ref{thm-two-counter}~(A)}

Let $M =(S,P,v)$ be a Markov chain such that $s \models \Psi$ for some $s \in S$. For every $k \in \{1,2\}$, let $T^k$ be the set of all $t \in S$ reachable from $s$ such that $t \not\models h^k$. It is easy to verify that the conditions of Theorem~\ref{thm-area} are satisfied for both $T^1$ and $T^2$, where  $\vec{v}^1[t]$ and $\vec{v}^2[t]$ play the role of $\vec{v}[t]$, respectively. 

We show that $s$ simulates $\M_1 \times_I \M_2$. Clearly, $s$ represents the configuration $(1,0,0)$ because $s \models \bInit^1 \wedge \bInit^2$. Let $t$ be a state reachable from $s$ such that $t$ represents a configuration $(j,n_1,n_2)$. Let $n_1',n_2' \in \N$ be the (unique) counter values in a successor configuration of $(j,n_1,n_2)$, and let $L$ be the set of all $j'$ such that $(j,n_1,n_2) \leadsto (j',n_1',n_2')$. 

Observe that  $t \models \Simulate^1 \wedge \Simulate^2$ and hence $t \models \NStep^1_{i,\ell_j} \wedge \NStep^2_{i',\ell_j}$ for some $i,i' \in \{0,\ldots,4\}$. Let $t'$ be an immediate successor of~$t$ such that $t' \models \ell^1_{j'} \wedge \ell^2_{j'}$ for some $j' \leq m$. Then $j' \in L$ by the definition of $\NStep_{i,\ell}^k$. Furthermore, at least one such $t'$ must exist because $t \models \LPass$. By using the arguments of Section~\ref{sec-prop-one-counter-unbounded}, we obtain that $\vec{v}^1[t'] = \sigma^{n'_1}(\vec{\kappa})$ and $\vec{v}^2[t'] = \sigma^{n'_2}(\vec{\kappa})$. Hence, $t'$ represents a successor configuration of $(j,n_1,n_2)$. Also observe that if $t''$ is an immediate successor of $t$ satisfying the formula $\bigwedge_{j=1}^m \neg(\ell_j^1 \wedge \ell_j^2)$, then all states reachable from $t''$ also satisfy this formula.

\subsubsection{A Proof of Theorem~\ref{thm-two-counter}~(B)}

Let $\omega = D_0,D_1,\ldots$ be a computation of $\M_1 \times_I \M_2$. If $\omega$ is periodic, we fix $\alpha,\beta$ such that $\alpha < \beta$ and the computations $D_{\alpha-1},D_{\alpha},D_{\alpha+1},\ldots$ and $D_{\beta-1},D_{\beta},D_{\beta+1},\ldots$ are the same. If $\omega$ is not periodic, then $\beta = \infty$ and $\alpha$ is undefined. 

For every configuration $D_i = (j,n_1,n_2)$ of $\omega$, let $C_i^1 = (j,n_1)$ and $C_i^2 = (j,n_2)$ be the corresponding configurations of $\M_1$ and $\M_2$. Furthermore, we define the infinite sequences $\omega^1 = C_0^1,C_1^1,C_2^1,\ldots$ and $\omega^2 = C_0^2,C_1^2,C_2^2,\ldots$. Note that $\omega_1$ and $\omega_2$ are \emph{not} necessarily computations of $\M_1$ and $\M_2$. However, for all $k \in \{1,2\}$ and $i \in \N$, we have that if $C_i^k = (j,n)$ and $C_{i+1}^k = (j',n')$, then there is $j'' \leq m$ such that $(j,n) \mapsto (j'',n')$ is a computational step of $\M_k$. In other words, $n'$ is obtained from $n$ by executing $\Ins_j$ in $\M_k$.  


% Furthermore, for $k \in \{1,2\}$, we define an infinite sequence $\omega_k = D_0^k,D_1^k,\ldots$ of configurations of $\M_k$ inductively as follows:
% \begin{itemize}
%     \item $D_0^k = (1,0)$;
%     \item if $C_i = (j,n_1,n_2)$ $C_i = (j,n_1,n_2)$ and where $j \in I_k$, then 
% \end{itemize} 


We construct a Markov chain $M = (S,P,v)$ and a state $s \in S$ such that $s \models \Psi$ and $s$ covers $\omega$. If $\beta < \infty$, then $S$ is finite.

The states of $S$ are tuples of the form $t = [\iota,\calL_1,\calL_2,n_1,n_2]$ where $\iota \in \{i \in \N \mid 0 \leq i < \beta\} \cup \{\star\}$, $\calL_1,\calL_2 \subseteq \A$, and $n_1,n_2 \in \N \cup \{\star\}$. The set $v(t)$ of atomic propositions satisfied in $t$ is $\{p^1 \mid p \in \calL_1\} \cup \{p^2 \mid p \in \calL_2\}$. 

Each state $t = [\iota,\calL_1,\calL_2,n_1,n_2]$ of $S$ determines two \emph{projections} $t_1 = [\iota,\calL_1,n_1]$ and $t_2 = [\iota,\calL_2,n_2]$. Conversely, for all $u_1 = [\iota,\calL_1,n_1]$ and $u_2 = [\iota,\calL_2,n_2]$ where $\iota,\calL_1,\calL_2,n_1,n_2$ satisfy the conditions of the previous paragraph we define a tuple $u_1 \uplus u_2 = [\iota,\calL_1,\calL_2,n_1,n_2]$.


The Markov chain $M$ is the least Markov chain $M'$ such that $s = [0,\{a,r_0,\ell_1\},\{a,r_0,\ell_1\},0,0]$ is a state of $M'$, and if $t$ is a state of $M'$, then $M'$ contains all immediate successors of $t$ defined by the rules given below. The rules are designed so that for every $t \in S$, the immediate successors of the projections $t_1$ and $t_2$ are defined by the rules of Section~\ref{sec-proof-prop-one-counter-bounded} where $\M_1$ and $\M_2$ are used as the underlying one-counter Minsky machines, the infinite sequences $\omega_1$ and $\omega_2$ play the role of the fixed computation $\omega$, and the constants $\alpha$ and $\beta$ refer to the constants fixed above. Recall that $\omega$ is used only in Rule~I of Section~\ref{sec-proof-prop-one-counter-bounded}, and this rule makes a clear sense also for $\omega^1$ and $\omega^2$. Also recall that the set $\Succ(t_k)$ of all immediate successors of $t_k$ (where $k \in \{1,2\}$) satisfies precisely one of the following conditions:
\begin{itemize}
    \item $\Succ(t_k) = \{t_k\}$. This happens iff $t_k \models h$.
    \item $\Succ(t_k)$ contains precisely three states satisfying the propositions $a$, $b$, and $c$, respectively, such that the last state does not satisfy~$d \vee e$. These states are denoted by $\ta_k$, $\tb_k$, and $\tc_k$, respectively.
    \item $\Succ(t_k)$ has precisely four states; apart of $\ta_k$, $\tb_k$, and $\tc_k$, there is also the fourth state satisfying $d$ or $e$. This fourth state is denoted by $\te_k$.
\end{itemize}

\noindent
Now we can define the closure rules.
\smallskip

\noindent
\textbf{Rule A.} If $t = [k,\{x,r_i,\ell_j\},\{x',r_{i'},\ell_j\},n_1,n_2]$ where $x,x' \in \{a,b\}$, $i,i' \in \{0,\ldots,4\}$, then the immediate successors of $t$ are defined as follows. 
Let $t_1' \in \Succ(t_1)$ and $t_2' \in \Succ(t_2)$ be the unique states satisfying some proposition of $\Labels$. Observe that $t_1' = [k',\calL_1,n_1]$ and $t_2' = [k',\calL_2,n_2]$ where $\calL_1$ and $\calL_2$ contain the \emph{same} proposition of $\Labels$ (this follows immediately by inspecting Rule~I of Section~\ref{sec-proof-prop-one-counter-bounded} and the definitions of $\omega^1$ and $\omega^2$).  We put 
\[
  P(t,t_1' \uplus t_2') = \min\{P(t_1,t_1'),P(t_2,t_2')\}\,.
\]
Furthermore, 
\begin{itemize}
    \item if $P(t_1,t_1') > P(t_2,t_2')$, then 
    \[
       P(t,t_1' \uplus \tc_2) = P(t_1,t_1') - P(t_2,t_2');
    \] 
    \item if $P(t_2,t_2') > P(t_1,t_1')$, then 
    \[
        P(t,\tc_1 \uplus t_2') = P(t_2,t_2') - P(t_1,t_1');
    \] 
    \item for all $t_1'' \in \Succ(t_1)$ where $t_1'' \neq t_1'$ and $t_1'' \in \{\ta_1,\tb_1,\te_1\}$, 
    \[
        P(t,t_1'' \uplus \tc_2) = P(t_1,t_1'');
    \]
    \item for all $t_2'' \in \Succ(t_2)$ where $t_2'' \neq t_2'$ and $t_2'' \in \{\ta_2,\tb_2,\te_2\}$, 
    \[
        P(t,\tc_1 \uplus t_2'') = P(t_2,t_2'');
    \]
    \item finally, we put 
    \(
        P(t,\tc_1 \uplus \tc_2) = 1-s
    \)
    where $s$ is the sum of all $P(t,\cdot)$ defined above.
\end{itemize}
Note that $s < 1$ due to the constraints on $q$ and $\vec{\kappa}$ adopted in Section~\ref{sec-counter}.  
\smallskip

\noindent
\textbf{Rule~B.} If $t = [k,\calL_1,\calL_2,n_1,n_2]$ where $\calL_1 \cap \Labels \neq \emptyset$, \mbox{$\calL_2 \cap \Labels = \emptyset$}, and $h \not\in \calL_2$, then $\calL_1$ contains precisely one $r_i \in \{r_0,\ldots,r_4\}$, and we distinguish two subcases.
\smallskip

\noindent
\pmb{$n_1 = 0$}. Then
\begin{eqnarray*}
    P(t,[\star,\{h,a,S(r_i)\},\star] \uplus \tc_2) & = & \vec{\kappa}_1,\\ 
    P(t,[\star,\{h,b,S^2(r_i)\},\star] \uplus \tc_2) & = & \vec{\kappa}_2,\\
    P(t,[\star,\{h,c,S^2(r_i),e\},\star] \uplus \tc_2) & = & 1-q \,.
\end{eqnarray*}
Furthermore, for every $t_2'' \in \{\ta_2,\tb_2,\te_2\}$, we put
\begin{eqnarray*}
    P(t,[\star,\{h,c,S^2(r_i)\},\star] \uplus t_2'') & = & P(t_2,t_2'')\,.
\end{eqnarray*}
Finally, we put $P(t,[\star,\{h,c,S^2(r_i)\},\star] \uplus \tc_2)  =  1-s$
% \begin{eqnarray*}
%     P(t,(h,c,S^2(r_i)) \uplus \tc_2) & = & 1-s
% \end{eqnarray*}
where $s$ is the sum of all $P(t,\cdot)$ defined above.
\smallskip

\noindent
\pmb{$n > 0$}. Then
\begin{eqnarray*}
    P(t,[\star,\{a,S(r_i)\},n{-}1] \uplus \tc_2) & = & \sigma^n(\vec{\kappa})_1,\\ 
    P(t,[\star,\{h,b,S^2(r_i)\},\star] \uplus \tc_2) & = & \sigma^n(\vec{\kappa})_2,\\
    P(t,[\star,\{h,c,S^2(r_i),e\},\star] \uplus \tc_2) & = & 1-q\,.
\end{eqnarray*}
Furthermore, for every $t_2'' \in \{\ta_2,\tb_2,\te_2\}$, 
\begin{eqnarray*}
    P(t,[\star,\{h,c,S^2(r_i)\},\star] \uplus t_2'') & = & P(t_2,t_2'')\,.
\end{eqnarray*}
Finally, we put $P(t,[\star,\{h,c,S^2(r_i)\},\star] \uplus \tc_2)  =  1-s$
% \begin{eqnarray*}
%     P(t,(h,c,S^2(r_i)) \uplus \tc_2) & = & 1-s
% \end{eqnarray*}
where $s$ is the sum of all $P(t,\cdot)$ defined above.
\smallskip

\noindent
\textbf{Rule~C.} If $t = [k,\calL_1,\calL_2,n_1,n_2]$ where $\calL_2 \cap \Labels \neq \emptyset$, \mbox{$\calL_1 \cap \Labels = \emptyset$}, and $h \not\in \calL_1$, then the immediate successors of $t$ are defined similarly as in Rule~B (Rule~C is fully symmetric to Rule~B).
\smallskip

\noindent
\textbf{Rule~D.} If $t = [k,\calL_1,\calL_2,n_1,n_2]$ where $\calL_1 \cap \Labels = \emptyset$, $\calL_2 \cap \Labels = \emptyset$, $h \not\in \calL_1$, and $h \not\in \calL_2$, then the immediate successors or $t$ are defined as follows. For every 
$t_1'' \in \{\ta_1,\tb_1,\te_1\}$, 
\begin{eqnarray*}
    P(t, t_1'' \uplus \tc_2) & = & P(t_1,t_1'')\,.
\end{eqnarray*}
Similarly, for all $t_2'' \in \{\ta_2,\tb_2,\te_2\}$, 
\begin{eqnarray*}
    P(t, \tc_1 \uplus t_2'') & = & P(t_2,t_2'')\,.
\end{eqnarray*}
Finally, $P(t, \tc_1 \uplus \tc_2) = 1 -s$, where $s$ is the sum of all $P(t,\cdot)$ above.
\smallskip

\noindent
\textbf{Rule~E.} If $t = [k,\calL_1,\calL_2,n_1,\star]$ where $h \not\in \calL_1$ and $h\in \calL_2$, then
\(
     P(t, t_1' \uplus t_2) = P(t_1,t_1')   
\)
for all $t_1' \in \Succ(t_1)$.
\smallskip 

\noindent
\textbf{Rule~F.} If $t = [k,\calL_1,\calL_2,n_1,\star]$ where $h \in \calL_1$ and $h \not\in \calL_2$, then
\(
    P(t, t_1 \uplus t_2') = P(t_2,t_2')   
\)
for all $t_2' \in \Succ(t_2)$.
\smallskip 

\noindent
\textbf{Rule~G.} If $t = [k,\calL_1,\calL_2,n_1,\star]$ where $h \in \calL_1$ and $h \in \calL_2$, then $P(t,t) =1$.
\smallskip 

If the computation $\omega$ is periodic, then the constructed Markov chain~$M$ has finitely many states. A routine check (similar to the one performed in the proof of Theorem~\ref{thm-one-counter}~(B)) reveals that the state $s = [0,\{a,r_0,\ell_1\},\{a,r_0,\ell_1\},0,0]$ satisfies $\Psi$ and covers the computation $\omega$.



